Forget-free Continual Learning with Soft-Winning SubNetworks

Inspired by Regularized Lottery Ticket Hypothesis (RLTH), which states that competitive smooth (non-binary) subnetworks exist within a dense network in continual learning tasks, we investigate two proposed architecture-based continual learning methods which sequentially learn and select adaptive binary- (WSN) and non-binary Soft-Subnetworks (SoftNet) for each task. WSN and SoftNet jointly learn the regularized model weights and task-adaptive non-binary masks of subnetworks associated with each task whilst attempting to select a small set of weights to be activated (winning ticket) by reusing weights of the prior subnetworks. Our proposed WSN and SoftNet are inherently immune to catastrophic forgetting as each selected subnetwork model does not infringe upon other subnetworks in Task Incremental Learning (TIL). In TIL, binary masks spawned per winning ticket are encoded into one N-bit binary digit mask, then compressed using Huffman coding for a sub-linear increase in network capacity to the number of tasks. Surprisingly, in the inference step, SoftNet generated by injecting small noises to the backgrounds of acquired WSN (holding the foregrounds of WSN) provides excellent forward transfer power for future tasks in TIL. SoftNet shows its effectiveness over WSN in regularizing parameters to tackle the overfitting, to a few examples in Few-shot Class Incremental Learning (FSCIL).

==> 1_abstract.tex <==
\begin{abstract}%v 
Inspired by \emph{Regularized Lottery Ticket Hypothesis (RLTH)}, which states that competitive smooth (non-binary) subnetworks exist within a dense network in continual learning tasks, we investigate two proposed architecture-based continual learning methods which sequentially learn and select adaptive binary- (WSN) and non-binary Soft-Subnetworks (SoftNet) for each task. WSN and SoftNet jointly learn the regularized model weights and task-adaptive non-binary masks of subnetworks associated with each task whilst attempting to select a small set of weights to be activated (winning ticket) by reusing weights of the prior subnetworks. Our proposed WSN and SoftNet are inherently immune to catastrophic forgetting as each selected subnetwork model does not infringe upon other subnetworks in Task Incremental Learning (TIL). In TIL, binary masks spawned per winning ticket are encoded into one N-bit binary digit mask, then compressed using Huffman coding for a sub-linear increase in network capacity to the number of tasks. Surprisingly, in the inference step, SoftNet generated by injecting small noises to the backgrounds of acquired WSN (holding the foregrounds of WSN) provides excellent forward transfer power for future tasks in TIL. SoftNet shows its effectiveness over WSN in regularizing parameters to tackle the overfitting, to a few examples in Few-shot Class Incremental Learning (FSCIL). 
\end{abstract}



==> 8_acknowledge.tex <==
\IEEEraisesectionheading{\section{Acknowledgement}}
This work was partly supported by Institute for Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (2021-0-01381) and partly supported by the IITP grant (2022-0-00184).

%This work was partly supported by Institute for Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (2021-0-01381) and partly supported by the IITP grant (2022-0-00184, Development and Study of AI Technologies to Inexpensively Conform to Evolving Policy on Ethics).

%This work was partly supported by Institute for Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (2021-0-01381, Development of Causal AI through Video Understanding and Reinforcement Learning, and Its Applications to Real Environments) and partly supported by the IITP grant (2022-0-00184, Development and Study of AI Technologies to Inexpensively Conform to Evolving Policy on Ethics).

%This work was partly supported by Institute for Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (2021-0-01381, Development of Causal AI through Video Understanding and Reinforcement Learning, and Its Applications to Real Environments) and partly supported by the IITP grant (2022-0-00184, Development and Study of AI Technologies to Inexpensively Conform to Evolving Policy on Ethics).

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> materials/3_concept_comparison.tex <==
\begin{figure*}[t]
  \small
  \centering
  \vspace{-0.6in}
  \includesvg[width=0.8\linewidth]{./images/concept_comparison.svg}\\
  \vspace{-0.5in}\caption{\small \textbf{Concept Comparison} (a) Piggyback \cite{mallya2018piggyback}, and SupSup \cite{wortsman2020supermasks} find the optimal binary mask on a fixed backbone network a given task (b) PackNet \cite{mallya2018packnet} and CLNP \cite{golkar2019continual} forces the model to reuse all features and weights from previous subnetworks which causes bias in transfer of knowledge (c) APD selectively reuse and dynamically expand the full network (d) Our proposed method selectively reuse and dynamically expand subnetworks within a full network. Green edges are re-used weights}
  \label{fig:concept_comparison}
\end{figure*}


==> materials/4_concept_figure.tex <==
\begin{figure*}[t]
  \small
  \centering
  \includesvg[width=0.8\linewidth]{images/method.svg}\\
  \vspace{-0.5in}\caption{\textbf{An illustration of Wining Subnetworks (WSN).} \modified{+ descriptions to explain this figure. [FIGURE TO BE REPLACED]}}
  \label{fig:concept_figure}
\end{figure*}


==> materials/5_acc_reused_per_tasks.tex <==
\begin{figure} %[htbp]
    \centering
    \setlength{\tabcolsep}{-7pt}{%
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{cc}
    
    \includegraphics[height=2.96cm,trim={0.3cm 0.1cm 0.1cm 0.1cm},clip]{images/exper_diagram.pdf} &\;\; 
    \includegraphics[height=2.96cm,trim={0.1cm 0.1cm 0.1cm 0.1cm},clip]{images/avg_acc_csnb_cifar100_10_c0.5.pdf} \\
    \end{tabular}}
    
    \caption{\textbf{Reused Weight Performances on CIFAR-100 Split:} (left) A diagram to explain a dense network of reused weights, (right) An average accuracy of reused weights; the most significant forgetting occurs from weights without reused per task; the significance of weights reused for all tasks gets lower as the number of tasks increases; In task 5, all used weights seem to be enough to infer all CIFAR-100 Split tasks since the weights reused per task catch up with the task performance.}
    \vspace{9cm} 
  \label{fig:reused_w_accuracy}
\end{figure}

==> materials/5_hyperparam_sweep.tex <==
\begin{figure*}[ht]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cc}
    % \includegraphics[height=3.cm]{images/5_per_task_acc_pmnist.pdf}&
    \includegraphics[height=3.cm]{images/5_per_task_acc_cifar.pdf}&
    \includegraphics[height=3.cm]{images/5_per_task_acc_5DATA.pdf} \\
    % \multicolumn{1}{c}{(a) PMNIST-MLP} & 
    \multicolumn{1}{c}{(b) SplitCIFAR100-AlexNet} &
    \multicolumn{1}{c}{(c) 5 Dataset-ResNet18}\\
    \end{tabular}}
    \caption{\footnotesize \textbf{Per task accuracy over varying $c\%$}}
    \label{fig:main_plot}
\end{figure*}

==> materials/5_main_conf_TinyImageNet.tex <==
\begin{figure}[h]
    \centering
    \vspace{-0.1in}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    % we prepare the figure 
    \includegraphics[width=0.5\columnwidth]{images/4_confusion/tinyimagenet/tinyimagenet_hard0.05.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/4_confusion/tinyimagenet/tinyimagenet_soft0.05.pdf} \\
    \small (a) WSN, $c = 5\%$ & \small (b) SoftNet, $c = 5\%$ \\
    \includegraphics[width=0.5\columnwidth]{images/4_confusion/tinyimagenet/tinyimagenet_hard0.7.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/4_confusion/tinyimagenet/tinyimagenet_soft0.7.pdf} \\
    \small (c) WSN, $c = 70\%$  & \small (d) SoftNet, $c = 70\%$
    \end{tabular}}
    \caption{\textbf{Average Confusion Matrix} on TinyImageNet WSN / SoftNet with $c = 3\%$ and $c = 70\%$.}
    \label{fig:main_conf_hard_soft_wsn_tiny}
    \vspace{-0.12in}
\end{figure}

==> materials/5_main_conf_cifar100_sc.tex <==
\begin{figure}[h]
    \centering
    \vspace{-0.1in}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    % we prepare the figure 
    \includegraphics[width=0.5\columnwidth]{images/4_confusion/cifar100_100_sc/cifar100_100_sc_hard0.05.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/4_confusion/cifar100_100_sc/cifar100_100_sc_soft0.05.pdf} \\
    \small (a) WSN, $c = 5\%$ & \small (b) SoftNet, $c = 5\%$ \\
    \includegraphics[width=0.5\columnwidth]{images/4_confusion/cifar100_100_sc/cifar100_100_sc_hard0.7.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/4_confusion/cifar100_100_sc/cifar100_100_sc_soft0.7.pdf} \\
    \small (c) WSN, $c = 70\%$  & \small (d) SoftNet, $c = 70\%$
    \end{tabular}}
    \caption{\textbf{Average Confusion Matrix} on Cifar-100 Superclass. WSN / SoftNet with $c = 3\%$ and $c = 70\%$.}
    \label{fig:main_conf_hard_soft_wsn_cifar100_sc}
    \vspace{-0.12in}
\end{figure}

==> materials/5_main_conf_omniglot.tex <==
\begin{figure}[h]
    \centering
    \vspace{-0.1in}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    % we prepare the figure 
    \includegraphics[width=0.5\columnwidth]{images/4_confusion/omniglot/omniglot_hard0.05.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/4_confusion/omniglot/omniglot_soft0.05.pdf} \\
    \small (a) WSN, $c = 5\%$ & \small (b) SoftNet, $c = 5\%$ \\
    \includegraphics[width=0.5\columnwidth]{images/4_confusion/omniglot/omniglot_hard0.7.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/4_confusion/omniglot/omniglot_soft0.7.pdf} \\
    \small (c) WSN, $c = 70\%$  & \small (d) SoftNet, $c = 70\%$
    \end{tabular}}
    \caption{\textbf{Average Confusion Matrix} on Omniglot. WSN / SoftNet with $c = 3\%$ and $c = 70\%$.}
    \label{fig:main_conf_hard_soft_wsn_omniglot}
    \vspace{-0.12in}
\end{figure}

==> materials/5_main_confusion_cifar100_10.tex <==
\begin{figure}[ht]
    \centering
    %\setlength{\tabcolsep}{-10pt}{%
    %\begin{tabular}{cccc}
    %\includegraphics[height=3.6cm]{images/corr_binary_csnb_cifar100_10_seed1_capacity_0.05.pdf} &~
    %\includegraphics[height=3.6cm]{images/corr_binary_csnb_cifar100_10_seed1_capacity_0.1.pdf} &~ 
    %\includegraphics[height=3.6cm]{images/corr_binary_csnb_cifar100_10_seed1_capacity_0.3.pdf} &~
    %\includegraphics[height=3.6cm]{images/corr_binary_csnb_cifar100_10_seed1_capacity_0.5.pdf} \\ 
    %\small (a) $c=0.05$ & \small (b) $c=0.1$ & 
    %\small (c) $c=0.3$ & \small (d) $c=0.5$ \\
    %\end{tabular}
    %}

    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    % we prepare the figure 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_cifar100_10_seed1_capacity_0.05.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_cifar100_10_seed1_capacity_0.1.pdf} \\
    \small (a) $c=5\%$ & \small (b) $c=10\%$ \\
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_cifar100_10_seed1_capacity_0.3.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_cifar100_10_seed1_capacity_0.5.pdf} \\
    \small (c) $c=30\%$ & \small (d) $c=50\%$
    \end{tabular}}
    
    \caption{\footnotesize \textbf{Average Binary Map Correlation} on Sequence of CIFAR-100 Split Experiments: the binary maps get overlapped with prior ones as the number of tasks increases..}
    \label{fig:main_cifar100_conf}
\end{figure}

==> materials/5_main_confusion_cifar100_100.tex <==
\begin{figure}[ht]
    \centering
    %\setlength{\tabcolsep}{-10pt}{%
    %\begin{tabular}{cccc}
    %\includegraphics[height=3.57cm]%{images/corr_binary_csnb_cifar100_100_seed1_capacity_0.05.pdf} &~\;
    %\includegraphics[height=3.57cm]%{images/corr_binary_csnb_cifar100_100_seed1_capacity_0.1.pdf} &~\; 
    %\includegraphics[height=3.57cm]%{images/corr_binary_csnb_cifar100_100_seed1_capacity_0.3.pdf} &~\;
    %\includegraphics[height=3.57cm]%{images/corr_binary_csnb_cifar100_100_seed1_capacity_0.5.pdf} \\ 
    %\small (a) $c=0.05$ & \small (b) $c=0.1$ & 
    %\small (c) $c=0.3$ & \small (d) $c=0.5$ \\
    %\end{tabular}
    %}

    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    % we prepare the figure 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_cifar100_100_seed1_capacity_0.05.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_cifar100_100_seed1_capacity_0.1.pdf} \\
    \small (a) $c=5\%$ & \small (b) $c=10\%$ \\
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_cifar100_100_seed1_capacity_0.3.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_cifar100_100_seed1_capacity_0.5.pdf} \\
    \small (c) $c=30\%$ & \small (d) $c=50\%$
    \end{tabular}}
    
    \caption{\footnotesize \textbf{Average Binary Map Correlation} on Sequence of CIFAR-100 Superclass Experiments: the binary maps get overlapped with prior ones as the number of tasks increases.}
    \label{fig:main_cifar100sc_conf}
\end{figure}

==> materials/5_main_confusion_tinyimagenet.tex <==
\begin{figure}[ht]
    \centering
    %\setlength{\tabcolsep}{-9pt}{%
    %\begin{tabular}{cccc}
    %\includegraphics[height=3.53cm]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.05.pdf} &~~
    %\includegraphics[height=3.53cm]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.1.pdf} &~~
    %\includegraphics[height=3.53cm]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.3.pdf} &~~
    %\includegraphics[height=3.53cm]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.5.pdf} \\ 
    %\small (a) $c=0.05$ & \small (b) $c=0.1$ & 
    %\small (c) $c=0.3$ & \small (d) $c=0.5$ \\
    %\end{tabular}
    %}

    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    % we prepare the figure 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.05.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.1.pdf} \\
    \small (a) $c=5\%$ & \small (b) $c=10\%$ \\
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.3.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.5.pdf} \\
    \small (c) $c=30\%$ & \small (d) $c=50\%$
    \end{tabular}}

    \caption{\footnotesize \textbf{Average Binary Map Correlation} on Sequence of TinyImageNet Dataset Experiments: the binary maps get overlapped with prior ones as the number of tasks increases..}
    \label{fig:main_tinyimg_conf}
\end{figure}

==> materials/5_main_confusion_tinyimagenet2.tex <==
\begin{figure}[t]
    \centering
    \vspace{-0.1in}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    % we prepare the figure 
    \includegraphics[height=3.2cm]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.1.pdf} & 
    \includegraphics[height=3.2cm]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.5.pdf} \\
    
    \small (a) WSN, $c=0.1$  &\small (b) WSN, $c=0.5$
    
    %\vspace{-0.05in}
    %\multicolumn{2}{c}{\small (a) Per Task Accuracy over Varying $c$} &
    %\multicolumn{3}{c}{\small (b) \% Weights used per Layer over Increasing No. of Tasks}
    \end{tabular}}
    
    \caption{\footnotesize \textbf{Task-wise Binary Map Correlations} on TinyImageNet: $c=0.5$ WSN reused task weights more than $c=0.1$ ones as shown in higher correlation results than others.}
    \label{fig:main_confs_wsn_packnet}
    \vspace{-0.12in}
\end{figure}

==> materials/5_main_plot_supsup_wsn.tex <==
\begin{figure}[t]
    %\vspace{-0.1in}
    \centering
    \begin{adjustbox}{width=0.7\columnwidth}
    \includegraphics[height=6.0cm, trim={1.0cm 0.1cm 1.0cm 0.1cm},clip]{images/5_experiments/5_acc_pmnist_supsup_wsn.pdf}
    \end{adjustbox}
    %\vspace{-0.25in}
    \caption{\textbf{Comparisons of SupSup and WSN on PMNIST-250}.}
  \label{fig:supsup_wsn_pmnis250}
  %\vspace{-0.1in}
\end{figure}

==> materials/5_main_plots.tex <==
\begin{figure*}[ht]
    \centering
    \setlength{\tabcolsep}{-15pt}{%
-    \begin{tabular}{cccc}
    \includegraphics[height=3.5cm]{images/5_cf_cifar.pdf} &
    \includegraphics[height=3.5cm]{images/5_acc_vs_cap_pmnist.pdf} &
    \includegraphics[height=3.5cm]{images/5_acc_vs_cap_5data.pdf} &
    \includegraphics[height=3.5cm]{images/5_used_weights_vs_num_tasks.pdf} &
    % \includegraphics[height=3.5cm]{images/5_acc_vs_sparsity.pdf}
     \\
     \small (a) Catastrophic Forgetting &
    \multicolumn{2}{c}{\small (b) Accuracy over Model Size} &
    % \multicolumn{2}{c}{(b) Catastrophic Forgetting during training} \\
    \small(c) Scalability to Large No. of Tasks  
    \end{tabular}}
    \caption{\footnotesize \textbf{Performance}}
    \label{fig:main_plots}
\end{figure*}

==> materials/5_main_plots_2.tex <==
\begin{figure*}[ht]
    \centering
    \setlength{\tabcolsep}{-25pt}{%
    \begin{tabular}{ccccc}
    \includegraphics[height=3.5cm]{images/5_per_task_acc_cifar.pdf} &
    \includegraphics[height=3.5cm]{images/5_per_task_acc_5DATA.pdf} &
    \includegraphics[height=3.5cm]{images/5_per_layer_sparsity_pmnist.pdf} &
    \includegraphics[height=3.5cm]{images/5_per_layer_sparsity_cifar.pdf} &
    \includegraphics[height=3.5cm]{images/5_per_layer_sparsity_5DATA.pdf} \\
    %\includegraphics[height=3.5cm]{images/5_acc_vs_sparsity.pdf}
    \multicolumn{2}{c}{\small (a) Per Task Accuracy over Varying $c$} &
    \multicolumn{3}{c}{\small (b) \% Weights used per Layer over Increasing No. of Tasks} 
    \end{tabular}}
    \caption{\footnotesize \textbf{Performance}}
    \label{fig:main_plots2}
\end{figure*}

==> materials/5_main_plots_capacity.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cccc}
    
    \includegraphics[width=0.25\textwidth]{images/avg_all_capa_csnb_tiny_data.pdf} & 
    % \hspace{0.08in}
    \includegraphics[width=0.25\textwidth]{images/avg_layer_all_capa_csnb_tiny_data_c0.1_conv.pdf} &
    % \hspace{0.08in} 
    \includegraphics[width=0.25\textwidth]{images/avg_layer_all_capa_csnb_tiny_data_c0.1_conv_linear.pdf} & 
    % \hspace{0.08in}
    \includegraphics[width=0.25\textwidth]{images/avg_layer_all_capa_csnb_tiny_data_c0.1_linear.pdf} \\ 
    
    % plot captions
    \small (a) Capacities over $c$ & \small (b) Conv1 vs. Conv4 Layer &
    \small (c) Conv4 vs. Linear2 Layer & \small (d) Linear1 vs. Linear2 Layer \\
    %\includegraphics[width=\linewidth]{images/avg_all_capa_csnb_tiny_data.pdf} &
    %\includegraphics[width=\linewidth]{images/avg_layer_all_capa_csnb_tiny_data_c0.1_conv.pdf} \\ 
    %\small (a) Capacities over $c$ & \small (b) Layer-wise-Capacities: conv1 v.s. conv4 layers \\
    %\includegraphics[width=\linewidth]{images/avg_layer_all_capa_csnb_tiny_data_c0.1_conv_linear.pdf} &
    %\includegraphics[width=\linewidth]{images/avg_layer_all_capa_csnb_tiny_data_c0.1_linear.pdf} \\ 
    %\small (c) Layer-wise-Capacities: conv4 v.s. linear2 layers & \small (d) Layer-wise-Capacities: linear1 v.s. linear2 layesr \\
    %\multicolumn{2}{c}{\small (a) } & \multicolumn{3}{c}{\small (b)}
    \end{tabular}
    %\end{adjustbox}
    }
    \caption{\textbf{The 4 Conv \& 3 FC Layer-wise Average Capacities} on Sequence of TinyImageNet Dataset Experiments. (a) The proportion of reused weights per task depends on $c$ value, and the proportion of reused weights for all tasks tends to be decreasing, (b) The capacity of Conv4 with high variance is greater than Conv1 with low variance, and the Conv4 proportion of reused weights for all tasks are smaller than the Conv1, (c) The capacity of Conv4 with high variance is greater than Liner2 with low variance and the Conv4 proportion of reused weights for all tasks are smaller than the Linear2, and (d) The capacity of Linear1 is greater than Linear2 in the early task learning stage, and the Linear1 proportion of reused weights for all tasks are smaller than the Linear2 in the early task learning stage. From (b), (c), and (d), the proportion of reused weights per task tends to be progressively saturated to $c=0.1$ value.}
    
    \label{fig:main_tinyimg_all_capa_plots}
\end{figure*}

==> materials/5_main_plots_tinyimgnet.tex <==
\begin{figure*}[ht]
    \centering
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{ccccc}
    \includegraphics[width=0.33333\textwidth]{images/avg_acc_csnb_tiny_data.pdf}  & 
    % \hspace{0.6in}
    \includegraphics[width=0.33333\textwidth]{images/avg_comp_rate_csnb_tiny_data_huffman.pdf} &
    % \hspace{0.6in}
    \includegraphics[width=0.33333\textwidth]{images/avg_bit_capa_csnb_tiny_data_huffman.pdf} \\
    
    
    \small (a) Per Task Accuracy over $c$ & \small (b) N-Bit-wise-Compression Rate & \small (c) Progressive Capacities of Models
    
    %\multicolumn{2}{c}{\small (a) Per Task Accuracy over Varying $c$} &
    %\multicolumn{3}{c}{\small (b) \% Weights used per Layer over Increasing No. of Tasks}
    \end{tabular}}
    \caption{\footnotesize \textbf{Performances and Compressed Capacities} - Sequence of TinyImageNet Dataset Experiments. (a) The $c=0.1$ shows generalized performances over others, (b) With fixed $c=0.1$, we investigate the bit-wise Huffman compression rate and observe that as the number of bits to compress increases the average compression rate gets higher, and (c) We compared the model capacity with the model capacity + the compressed binary masks over varying bits. Within the 40-tasks, the 7-bits compressed capacities are the least increasing along with the $c=0.1$ model capacity.}
    \label{fig:app_main_tinyimg_plots}
\end{figure*}

==> materials/5_main_table.tex <==
\begin{table*}[t]
\tiny
\begin{center}
\caption{\small Performance comparison of the proposed method and other baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (Accuracy) and average forgetting (Forgetting) across $5$ independent runs. CF indicates that the method suffers from the catastrophic forgetting. The best results are highlighted in bold. Values with $\dagger$ $~$ denote reported performances from \cite{Saha2021}. PackNet~\cite{mallya2018packnet} is baseline.}

\begin{adjustbox}{width=1.0\textwidth}
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Method}}&\multicolumn{2}{c}{\textbf{Permuted MNIST}} & \multicolumn{2}{c}{\textbf{Split CIFAR-100}} & \multicolumn{2}{c}{\textbf{5 Datasets}} \\


\midrule
& CF & Accuracy & Capacity Used & Accuracy & Capacity Used & Accuracy & Capacity Used\\
\midrule
STL & $\bsy\times$ &
{\scriptsize 97.6} ($\pm$ 0.10) & {\scriptsize 1000.0} \%&
{\scriptsize 70.9} ($\pm$ 0.38) & {\scriptsize 1000.0} \%&
{\scriptsize 90.7} ($\pm$ 0.53) & {\scriptsize 500.0} \%\\
 \midrule
FINETUNE&  \checkmark &
{\scriptsize 62.5} ($\pm$ 2.96) & {\scriptsize 100.0} \%&
{\scriptsize 13.2} ($\pm$ 0.54) & {\scriptsize 100.0} \%&
{\scriptsize 36.8} ($\pm$ 2.25) & {\scriptsize 100.0} \%\\
HAT~\cite{Serra2018} &  \checkmark &
{\scriptsize -}  & {\scriptsize -} &
{\scriptsize 72.0} $\dagger$ & {\scriptsize 100.0} \%&
{\scriptsize 88.6} $\dagger$ & {\scriptsize 100.0} \%\\
% APD~\cite{Yoon2020}  & \checkmark &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%\\

AGS-CL~\cite{Jung2020} & \checkmark &
{\scriptsize 91.1} ($\pm$ 0.71) & {\scriptsize 100.0} \%&
{\scriptsize 49.6} ($\pm$ 1.89) & {\scriptsize 100.0} \%&
{\scriptsize -}  & -\\

GPM~\cite{Saha2021} & \checkmark &
% {\scriptsize 92.9} ($\pm$ 0.20) & {\scriptsize x.xx} \%&
{\scriptsize 93.9} $\dagger$ & {\scriptsize 100.0} \%&
{\scriptsize 72.5} $\dagger$ & {\scriptsize 100.0} \%&
{\scriptsize 91.3} $\dagger$ & {\scriptsize 100.0} \%\\
\cmidrule{1-8}
PackNet~\cite{mallya2018packnet}  & $\bsy\times$ &
%\textbf{{\scriptsize 95.9} ($\pm$ 0.05)} & {\scriptsize $~$ 96.8} \%& % 0.655 + 10*1/32
{\scriptsize 94.5} ($\pm$ 0.05) & {\scriptsize $~$ 72.1} \%& % 0.408 + 10*1/32
{\scriptsize 58.3} ($\pm$ 0.46) & {\scriptsize 131.2} \%& % 0.999 + 10*1/32
{\scriptsize 89.0} ($\pm$ 0.21) & {\scriptsize 115.4} \%\\ % 0.998 + 5 * 1/32
% LL-Ticket~\cite{longliveticket}  & $\bsy\times$ &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%\\
\cmidrule{1-8}
CST (Ours) $c=0.03$ & $\bsy\times$ &
{\scriptsize 92.7} ($\pm$ 0.06) & \textbf{{\scriptsize $~$ 37.4}} \%&
{\scriptsize 65.6} ($\pm$ 0.63) & \textbf{{\scriptsize $~$ 39.4}} \%&
{\scriptsize 90.1} ($\pm$ 0.10) & \textbf{{\scriptsize $~$ 24.2}} \%\\
CST (Ours) $c=0.1$ & $\bsy\times$ &
{\scriptsize 93.9} ($\pm$ 0.09) & {\scriptsize $~$ 46.3} \%&
{\scriptsize 72.2} ($\pm$ 0.36) & {\scriptsize $~$ 56.2} \%&
{\scriptsize 91.3} ($\pm$ 0.13) & {\scriptsize $~$ 39.9} \%\\
CST (Ours) $c=0.3$ & $\bsy\times$ &
{\scriptsize 94.7} ($\pm$ 0.07) & {\scriptsize $~$ 68.3} \%& \textbf{{\scriptsize 73.5} ($\pm$ 0.40)} & {\scriptsize $~$ 97.4} \%& \textbf{{\scriptsize 91.7} ($\pm$ 0.23)} & {\scriptsize $~$ 72.9} \%\\
CST (Ours) $c=0.5$ & $\bsy\times$ &
\textbf{{\scriptsize 94.8} ($\pm$ 0.02)} & {\scriptsize $~$ 88.9} \%& {\scriptsize 72.5 ($\pm$ 0.92)} & {\scriptsize 111.0} \%& {\scriptsize 91.5} ($\pm$ 0.13) & {\scriptsize $~$ 95.8} \%\\
\cmidrule{1-8}
MTL &$\bsy\times$& {\scriptsize 96.7 $\dagger$} & {\scriptsize 100.0} \%& {\scriptsize 79.6 $\dagger$} & {\scriptsize 100.0} \%& {\scriptsize 91.5 $\dagger$} & {\scriptsize 100.0} \%\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:main_table}
\end{center}
\end{table*}




==> materials/5_main_table_new.tex <==
\begin{table*}[ht]
\small
\begin{center}
\caption{\small Performance comparison of the proposed method and other baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (ACC), average capacity (CAP), and average backward transfer (BWT) across $5$ independent runs. CF indicates that the method suffers from the catastrophic forgetting. The best results are highlighted in bold. Values with $\dagger$ and * denote reported performances from \citet{Saha2021} and \citet{Yoon2020}. PackNet~\cite{mallya2018packnet} is set to baseline as a non-reused weight model.}

%\begin{adjustbox}{width=1.0\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Method}}&\multicolumn{3}{c}{\textbf{Permuted MNIST}}&
% \multicolumn{3}{c}{\textbf{Split CIFAR-100}}&
% \multicolumn{3}{c}{\textbf{Split CIFAR-100 Superclass}}&
\multicolumn{3}{c}{\textbf{5 Datasets}}&
\multicolumn{3}{c}{\textbf{Omniglot Rotation}} \\


\midrule
&CF&
ACC (\%)&CAP (\%)&BWT&
% ACC (\%)&CAP (\%)&BWT (\%)&
% ACC (\%)&CAP (\%)&BWT (\%)&
ACC (\%)&CAP (\%)&BWT&
ACC (\%)&CAP (\%)&BWT \\
\midrule
STL&$\bsy\times$&
% {97.6}~\scriptsize($\pm$ 0.10)&{1000.0} \%&&
% {70.9}~\scriptsize($\pm$ 0.38)&{1000.0} \%&&
% {90.7}~\scriptsize($\pm$ 0.53)&{500.0} \%&&
%&&&
%&&\\
{97.2}~\scriptsize($\pm$ 0.11)&{$~$ 1000.0}~\scriptsize($\pm$ 0.00)&-&
% {73.9}~\scriptsize($\pm$ 0.44)&{$~$ 1000}~\scriptsize($\pm$ 0.00)&{0.00}~\scriptsize($\pm$ 0.00)&
% {62.0}~\scriptsize($\pm$ 0.44)&{$~$ 2000}~\scriptsize($\pm$ 0.00)&{0.00}~\scriptsize($\pm$ 0.00)&
{93.4}~\scriptsize($\pm$ 0.12)&{$~$ 500.0}~\scriptsize($\pm$ 0.00)&-&
{82.1}~\scriptsize($\pm$ 0.08){\scriptsize*}&{$~$ 10000.0}~\scriptsize($\pm$ 0.00)& - \\
 \midrule
FINETUNE&\checkmark&
% {62.5}~\scriptsize($\pm$ 2.96)&{100.0} \%&&
% {13.2}~\scriptsize($\pm$ 0.54)&{100.0} \%&&
% {36.8}~\scriptsize($\pm$ 2.25)&{100.0} \%&&
%&&&
%&&\\
~{78.2}~\scriptsize($\pm$ 0.84)&{$~$ 100.0}~\scriptsize($\pm$ 0.00)&~~{-0.21}~\scriptsize($\pm$ 0.01)&
% {17.3}~\scriptsize($\pm$ 0.28)&{$~$ 100}~\scriptsize($\pm$ 0.00)&{-65.0}~\scriptsize($\pm$ 0.40)&
% {20.0}~\scriptsize($\pm$ 0.00)&{$~$ 100}~\scriptsize($\pm$ 0.00)&{-15.3}~\scriptsize($\pm$ 5.26)&
{80.1}~\scriptsize($\pm$ 0.74)&{$~$ 100.0}~\scriptsize($\pm$ 0.00)&{-0.17}~\scriptsize($\pm$ 0.01)&
{44.5}~\scriptsize($\pm$ 1.68)&{$~$ 100.0}~\scriptsize($\pm$ 0.00)&{-0.45}~\scriptsize($\pm$ 0.02) \\


EWC~\cite{Kirkpatrick2017}&\checkmark&~{92.0}~\scriptsize($\pm$ 0.60)&~~{100.0}~\scriptsize($\pm$ 0.00)&~{-0.03}~\scriptsize($\pm$ 0.00)&
% {xx.x}~\scriptsize($\pm$ x.xx)&{x.xx} \%&{-}~\scriptsize($\pm$ -)&
% {xx.x}~\scriptsize($\pm$ x.xx)&{x.xx} \%&{-}~\scriptsize($\pm$ -)&
~~{88.6}~\scriptsize($\pm$ 0.26)$^\dagger$&~~~~{100.0}~\scriptsize($\pm$ 0.00)$^\dagger$&~~{-0.04}~\scriptsize($\pm$ 0.01)$^\dagger$&~~{68.7}~\scriptsize($\pm$ 1.92){\scriptsize*}&~~~~{100.0}~\scriptsize($\pm$ 0.00){\scriptsize*}&{-} \\




HAT~\cite{Serra2018}&\checkmark&
% {-}&{-}&&
% {72.0} $^\dagger$&{100.0} \%&&
% {88.6} $^\dagger$&{100.0} \%&&
%&&&
%&&\\
{-}&{-}&{-}&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
~~{91.3}~\scriptsize($\pm$ 0.18)$^\dagger$&~~~~{100.0}~\scriptsize($\pm$ 0.00)$^\dagger$&~~{-0.03}~\scriptsize($\pm$ 0.00)$^\dagger$&
{-}&{-}&{-} \\
% APD~\cite{Yoon2020}&\checkmark&
% {xx.x}~\scriptsize($\pm$ x.xx)&{x.xx} \%&{-}~\scriptsize($\pm$ -)&
% % {xx.x}~\scriptsize($\pm$ x.xx)&{x.xx} \%&{-}~\scriptsize($\pm$ -)&
% % {xx.x}~\scriptsize($\pm$ x.xx)&{x.xx} \%&{-}~\scriptsize($\pm$ -)&
% {xx.x}~\scriptsize($\pm$ x.xx)&{x.xx} \%&{-}~\scriptsize($\pm$ -)&
% {81.2}~\scriptsize($\pm$ 0.53) {*}&{943}~\scriptsize($\pm$ 0.00)&{-}~\scriptsize($\pm$ -) \\



% AGS-CL~\cite{Jung2020}&\checkmark&
% % {91.1}~\scriptsize($\pm$ 0.71)&{100.0} \%&&
% % {49.6}~\scriptsize($\pm$ 1.89)&{100.0} \%&&
% % {-}&-&&
% %&&&
% %&&\\
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% % {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% % {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -) \\
GPM~\cite{Saha2021}&\checkmark&
% {92.9}~\scriptsize($\pm$ 0.20)&{x.xx} \%&
% {93.9} $^\dagger$&{100.0} \%&&
% {72.5} $^\dagger$&{100.0} \%&&
% {91.3} $^\dagger$&{100.0} \%&&
%&&&
%&&\\
{95.0}~\scriptsize($\pm$ 0.07)&{$~$ 100.0}~\scriptsize($\pm$ 0.00)&{-0.02}~\scriptsize($\pm$ 0.01)&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
~~{91.2}~\scriptsize($\pm$ 0.20)$^\dagger$&{$~$ 100.0}~\scriptsize($\pm$ 0.00)&~~{-0.01}~\scriptsize($\pm$ 0.00)$^\dagger$&
{85.24}~\scriptsize($\pm$ 0.38)&{$~$ 100.0}~\scriptsize($\pm$ 0.00) &{0.01}~\scriptsize($\pm$ 0.00) \\
\midrule
PackNet~\cite{mallya2018packnet}&$\bsy\times$&
%\textbf{{95.9}~\scriptsize($\pm$ 0.05)}&{$~$ 96.8} \%&% 0.655 + 10*1/32
% {94.5}~\scriptsize($\pm$ 0.05)&{$~$ 72.1} \%&&% 0.408 + 10*1/32
% {58.3}~\scriptsize($\pm$ 0.46)&{131.2} \%&&% 0.999 + 10*1/32
% {89.0}~\scriptsize($\pm$ 0.21)&{115.4} \%&&% 0.998 + 5 * 1/32 
%&&&
%&&\\ 
{95.5}~\scriptsize($\pm$ 1.29)&{$~$ 125.6}~\scriptsize($\pm$ 0.00)&{0.00}~\scriptsize($\pm$ 0.00)&% 0.9437 + 10*1/32 % plus per-task mask
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
{92.8}~\scriptsize($\pm$ 0.12)&{$~$ 82.8}~\scriptsize($\pm$ 0.00)&{0.00}~\scriptsize($\pm$ 0.00)& % 67.2 + 100*5/32 = 82.8
% 67.2 + 100*5/32*(1-0.78) = 70.7
% {23.8}~\scriptsize($\pm$ 1.11)&{$~$ 375.9}~\scriptsize($\pm$ 0.00)&{0.00}~\scriptsize($\pm$ 0.00) \\ % 63.4 + 100*100/32 = 375.9
{30.7}~\scriptsize($\pm$ 1.50)&{$~$ 399.2}~\scriptsize($\pm$ 0.00)&{0.00}~\scriptsize($\pm$ 0.00) \\ % 86.74 + 100*100/32 = 399.2
% 86.74 + 100*100*(1-0.78)/32 = 155.5
% LL-Ticket~\cite{longliveticket}&$\bsy\times$&
% {xx.x}~\scriptsize($\pm$ x.xx)&{$~$ x.xx} \%&
% {xx.x}~\scriptsize($\pm$ x.xx)&{$~$ x.xx} \%&
% {xx.x}~\scriptsize($\pm$ x.xx)&{$~$ x.xx} \%\\
\midrule
WSN, $c=0.03$&$\bsy\times$&% need to add per-task sparsity
{95.0}~\scriptsize($\pm$ 0.11)&\textbf{{$~$ 16.6}~\scriptsize($\pm$ 0.06)}&{0.00}~\scriptsize($\pm$ 0.00)&% 13.1 + 100*(1-0.78)*10/32 = 16.57 $\pm$ 0.06
% {71.0}~\scriptsize($\pm$ 0.56)&\textbf{{$~$ 11.7}~\scriptsize($\pm$ 0.25)}&{0.00}~\scriptsize($\pm$ 0.00)&
% {62.5}~\scriptsize($\pm$ 0.40)&\textbf{{$~$ 10.4}~\scriptsize($\pm$ 0.24)}&{0.00}~\scriptsize($\pm$ 0.00)&
%{90.6}~\scriptsize($\pm$ 0.65)&\textbf{{$~$ 8.67}~\scriptsize($\pm$ 0.06)}&{0.00}~\scriptsize($\pm$ 0.00)&
{90.6}~\scriptsize($\pm$ 0.65)&\textbf{{$~$ 12.1}~\scriptsize($\pm$ 0.06)}&{0.00}~\scriptsize($\pm$ 0.00)& % 8.7 + 100*(1-0.78)*5/32 = 12.1 $\pm$ 0.082
{80.7}~\scriptsize($\pm$ 2.60)&\textbf{{$~~~$ 75.9}~\scriptsize($\pm$ 1.24)}&{0.00}~\scriptsize($\pm$ 0.00) \\ % 7.1 + 100*(1-0.78)*100/32 = 75.9 $\pm$ 1.24

WSN, $c=0.05$&$\bsy\times$&% need to add per-task sparsity
{95.6}~\scriptsize($\pm$ 0.15)&{$~$ 22.9}~\scriptsize($\pm$ 0.33)&{0.00}~\scriptsize($\pm$ 0.00)& % 19.5 + 100*(1-0.78)*10/32 = 22.9
% {72.4}~\scriptsize($\pm$ 0.44)&{$~$ 18.3}~\scriptsize($\pm$ 0.54)&{0.00}~\scriptsize($\pm$ 0.00)&
% {63.1}~\scriptsize($\pm$ 0.16)&{$~$ 14.9}~\scriptsize($\pm$ 0.63)&{0.00}~\scriptsize($\pm$ 0.00)&
{91.6}~\scriptsize($\pm$ 0.21)&{$~$ 17.3}~\scriptsize($\pm$ 0.25)&{0.00}~\scriptsize($\pm$ 0.00)& % 13.8 + 100*(1-0.78)*5/32 = 17.3
\textbf{{87.3}~\scriptsize($\pm$ 0.72)}&{$~~~$ 79.8}~\scriptsize($\pm$ 1.19)&{0.00}~\scriptsize($\pm$ 0.00) \\ % 11.1 + 100*(1-0.78)*100/32 = 79.8

WSN, $c=0.1$&$\bsy\times$&% need to add per-task sparsity
{96.2}~\scriptsize($\pm$ 0.10)&{$~$ 37.2}~\scriptsize($\pm$ 0.44)&{0.00}~\scriptsize($\pm$ 0.00)& % 33.8 + 100*(1-0.78)*10/32 = 37.2
% {74.7}~\scriptsize($\pm$ 0.33)&{$~$ 32.7}~\scriptsize($\pm$ 0.75)&{0.00}~\scriptsize($\pm$ 0.00)&
% \textbf{{63.7}~\scriptsize($\pm$ 0.39)}&{$~$ 22.9}~\scriptsize($\pm$ 1.56)&\textbf{{0.00}~\scriptsize($\pm$ 0.00)}&
{92.7}~\scriptsize($\pm$ 0.12)&{$~$ 28.0}~\scriptsize($\pm$ 0.28)&{0.00}~\scriptsize($\pm$ 0.00)& % 24.6 + 100*(1-0.78)*5/32 = 28.0
{83.1}~\scriptsize($\pm$ 1.56)&{$~~~$ 83.1}~\scriptsize($\pm$ 1.61)&{0.00}~\scriptsize($\pm$ 0.00) \\ % 14.3 + 100*(1-0.78)*100/32 = 83.1

WSN, $c=0.3$&$\bsy\times$&% need to add per-task sparsity
\textbf{{96.5}~\scriptsize($\pm$ 0.06)}&{$~$ 73.6}~\scriptsize($\pm$ 0.50)&\textbf{{0.00}~\scriptsize($\pm$ 0.00)}& % 70.2 + 100*(1-0.78)*10/32 = 73.6
% {76.4}~\scriptsize($\pm$ 0.38)&{$~$ 73.1}~\scriptsize($\pm$ 0.81)&{0.00}~\scriptsize($\pm$ 0.00)&
% {63.4}~\scriptsize($\pm$ 0.26)&{$~$ 38.2}~\scriptsize($\pm$ 0.74)&{0.00}~\scriptsize($\pm$ 0.00)&
{93.2}~\scriptsize($\pm$ 0.32)&{$~$ 62.3}~\scriptsize($\pm$ 0.69)&{0.00}~\scriptsize($\pm$ 0.00)& % 58.9 + 100*(1-0.78)*5/32 = 62.3
{81.9}~\scriptsize($\pm$ 1.14)&{$~$ 102.2}~\scriptsize($\pm$ 0.89)&{0.00}~\scriptsize($\pm$ 0.00) \\ % 33.4 + 100*(1-0.78)*100/32 = 102.2

WSN, $c=0.5$&$\bsy\times$&% need to add per-task sparsity
{96.3}~\scriptsize($\pm$ 0.08)&{$~$ 94.3}~\scriptsize($\pm$ 0.31)&{0.00}~\scriptsize($\pm$ 0.00)& % 90.9 + 100*(1-0.78)*10/32 = 94.3
% \textbf{{76.5}~\scriptsize($\pm$ 0.39)}&{$~$ 92.2}~\scriptsize($\pm$ 0.75)&\textbf{{0.00}~\scriptsize($\pm$ 0.00)}&
% {63.4}~\scriptsize($\pm$ 0.17)&{$~$ 57.0}~\scriptsize($\pm$ 0.63)&{0.00}~\scriptsize($\pm$ 0.00)&
\textbf{{93.4}~\scriptsize($\pm$ 0.13)}&{$~$ 86.1}~\scriptsize($\pm$ 0.57)&{0.00}~\scriptsize($\pm$ 0.00)& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{79.8}~\scriptsize($\pm$ 2.16)&{$~$ 121.2}~\scriptsize($\pm$ 0.50)&{0.00}~\scriptsize($\pm$ 0.00) \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

% WSN, $c=0.7$&$\bsy\times$&% need to add per-task sparsity
% {96.3}~\scriptsize($\pm$ 0.08)&{$~$ 90.9}~\scriptsize($\pm$ 0.31)&{0.00}~\scriptsize($\pm$ 0.00)&
% % \textbf{{76.5}~\scriptsize($\pm$ 0.39)}&{$~$ 92.2}~\scriptsize($\pm$ 0.75)&\textbf{{0.00}~\scriptsize($\pm$ 0.00)}&
% % {63.4}~\scriptsize($\pm$ 0.17)&{$~$ 57.0}~\scriptsize($\pm$ 0.63)&{0.00}~\scriptsize($\pm$ 0.00)&
% \textbf{{93.4}~\scriptsize($\pm$ 0.13)}&{$~$ 82.7}~\scriptsize($\pm$ 0.57)&{0.00}~\scriptsize($\pm$ 0.00)&
% {79.8}~\scriptsize($\pm$ 2.16)&{$~$ 52.4}~\scriptsize($\pm$ 0.50)&{0.00}~\scriptsize($\pm$ 0.00) \\ % need to add (per-task)

% WSN, $c=0.9$&$\bsy\times$&% need to add per-task sparsity
% {96.3}~\scriptsize($\pm$ 0.08)&{$~$ 90.9}~\scriptsize($\pm$ 0.31)&{0.00}~\scriptsize($\pm$ 0.00)&
% % \textbf{{76.5}~\scriptsize($\pm$ 0.39)}&{$~$ 92.2}~\scriptsize($\pm$ 0.75)&\textbf{{0.00}~\scriptsize($\pm$ 0.00)}&
% % {63.4}~\scriptsize($\pm$ 0.17)&{$~$ 57.0}~\scriptsize($\pm$ 0.63)&{0.00}~\scriptsize($\pm$ 0.00)&
% \textbf{{93.4}~\scriptsize($\pm$ 0.13)}&{$~$ 82.7}~\scriptsize($\pm$ 0.57)&{0.00}~\scriptsize($\pm$ 0.00)&
% {79.8}~\scriptsize($\pm$ 2.16)&{$~$ 52.4}~\scriptsize($\pm$ 0.50)&{0.00}~\scriptsize($\pm$ 0.00) \\ % need to add (per-task)

\midrule
MTL&$\bsy\times$&
~~{96.7~\scriptsize($\pm$ 0.02)$^\dagger$}&{100.0}&{-}&
% {79.6 $^\dagger$}&{100.0} \%&{-}&
~~{91.5~\scriptsize($\pm$ 0.28)$^\dagger$}&{100.0}&{-}&
% {-}&{-} \%&{-}&
{81.2~\scriptsize($\pm$ 0.50)}&{100.0}&{-} \\
\bottomrule
\end{tabular}}
%\end{adjustbox}
\label{tab:main_table_new}
\end{center}
\end{table*}




==> materials/5_main_table_sota.tex <==
\begin{table*}[t]
\small
\begin{center}
\caption{\small  Performance comparisons of the proposed method and other state-of-the-art on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (ACC), average capacity (CAP), and average backward transfer (BWT) across $5$ independent runs with 5 seeds under the same experimental setup \cite{deng2021flattening}. CF indicates that the method suffers from the catastrophic forgetting. The best results are highlighted in bold. Also, $\dagger$ $~$ denotes results reported from \cite{deng2021flattening}.}

\begin{adjustbox}{width=1.0\textwidth}
\begin{tabular}{l|c|ccc|ccc|ccccc}
\toprule
\multicolumn{2}{c}{\textbf{Method}}&\multicolumn{3}{c}{\textbf{CIFAR-100 Split}} & \multicolumn{3}{c}{\textbf{CIFAR-100 Superclass}} & \multicolumn{3}{c}{\textbf{TinyImageNet}} \\


\midrule
& CF & ACC (\%) & CAP (\%) & BWT (\%) & ACC (\%) & CAP (\%) & BWT (\%) & ACC (\%) & CAP (\%) & BWT (\%)  \\
\midrule
La-MaML \cite{gupta2020maml} & \checkmark  & 71.37~\scriptsize($\pm$ 0.67)$^\dagger$ & 100.0 & -5.39~\scriptsize($\pm$ 0.53)$^\dagger$ & 54.44~\scriptsize($\pm$ 1.36)$^\dagger$ & 100.0  & -6.65~\scriptsize($\pm$ 0.85)$^\dagger$ & 66.90~\scriptsize($\pm$ 1.65)$^\dagger$ & 100.0  & -9.13~\scriptsize($\pm$ 0.90)$^\dagger$  \\
GPM \cite{Saha2021} & \checkmark   & 73.18~\scriptsize($\pm$ 0.52)$^\dagger$ & 100.0 & -1.17~\scriptsize($\pm$ 0.27)$^\dagger$ & 57.33~\scriptsize($\pm$ 0.37)$^\dagger$ & 100.0  & -0.37~\scriptsize($\pm$ 0.12)$^\dagger$ & 67.39~\scriptsize($\pm$ 0.47)$^\dagger$ & 100.0  & ~\textbf{1.45}~\scriptsize($\pm$ \textbf{0.22})$^\dagger$  \\
FS-DGPM \cite{deng2021flattening} & \checkmark  & 74.33~\scriptsize($\pm$ 0.31)$^\dagger$ & 100.0 & -2.17~\scriptsize($\pm$ 0.17)$^\dagger$ & 58.81~\scriptsize($\pm$ 0.34)$^\dagger$  & 100.0  & -2.97~\scriptsize($\pm$ 0.35)$^\dagger$ & 70.41~\scriptsize($\pm$ 1.30)$^\dagger$  & 100.0  & -2.11~\scriptsize($\pm$ 0.84)$^\dagger$ \\

\midrule

%WSN, $c=0.03$ & $\bsy \times$ & 70.65~\scriptsize($\pm$ 0.36) & \textbf{11.69}~\scriptsize($\pm$ \textbf{0.25}) & 0.0~\scriptsize($\pm$ 0.0) & 54.99~\scriptsize($\pm$ 0.71) & ~~\textbf{8.55}~\scriptsize($\pm$ \textbf{0.22})  & 0.0~\scriptsize($\pm$ 0.0) & 68.72~\scriptsize($\pm$ 1.63) & ~~\textbf{9.69}~\scriptsize($\pm$ \textbf{0.21})  & 0.0~\scriptsize($\pm$ 0.0)  \\
WSN, $c=0.03$ & $\bsy \times$ & 70.65~\scriptsize($\pm$ 0.36) & \textbf{18.56}~\scriptsize($\pm$ \textbf{0.25}) & 0.0~\scriptsize($\pm$ 0.0) & 54.99~\scriptsize($\pm$ 0.71) & \textbf{22.30}~\scriptsize($\pm$ \textbf{0.22})  & 0.0~\scriptsize($\pm$ 0.0) & 68.72~\scriptsize($\pm$ 1.63) & \textbf{37.19}~\scriptsize($\pm$ \textbf{0.21})  & 0.0~\scriptsize($\pm$ 0.0)  \\

%WSN, $c=0.05$ & $\bsy \times$ & 72.44~\scriptsize($\pm$ 0.27) & 18.22~\scriptsize($\pm$ 0.42) & 0.0~\scriptsize($\pm$ 0.0) & 57.99~\scriptsize($\pm$ 1.34) & 13.62~\scriptsize($\pm$ 0.33)  & 0.0~\scriptsize($\pm$ 0.0) & 71.22~\scriptsize($\pm$ 0.94) & 14.48~\scriptsize($\pm$ 0.52)  & 0.0~\scriptsize($\pm$ 0.0)  \\
WSN, $c=0.05$ & $\bsy \times$ & 72.44~\scriptsize($\pm$ 0.27) & 25.09~\scriptsize($\pm$ 0.42) & 0.0~\scriptsize($\pm$ 0.0) & 57.99~\scriptsize($\pm$ 1.34) & 27.37~\scriptsize($\pm$ 0.33)  & 0.0~\scriptsize($\pm$ 0.0) & 71.22~\scriptsize($\pm$ 0.94) & 41.98~\scriptsize($\pm$ 0.52)  & 0.0~\scriptsize($\pm$ 0.0)  \\


%WSN, $c=0.1$ & $\bsy \times$ & 74.55~\scriptsize($\pm$ 0.47) & 33.00~\scriptsize($\pm$ 0.62) & 0.0~\scriptsize($\pm$ 0.0) & 60.45~\scriptsize($\pm$ 0.37) & 24.80~\scriptsize($\pm$ 0.20)  & 0.0~\scriptsize($\pm$ 0.0) & \textbf{71.96}~\scriptsize($\pm$ \textbf{1.41}) & 21.15~\scriptsize($\pm$ 3.03)  & 0.0~\scriptsize($\pm$ 0.0)  \\
WSN, $c=0.1$ & $\bsy \times$ & 74.55~\scriptsize($\pm$ 0.47) & 39.87~\scriptsize($\pm$ 0.62) & 0.0~\scriptsize($\pm$ 0.0) & 60.45~\scriptsize($\pm$ 0.37) & 38.55~\scriptsize($\pm$ 0.20)  & 0.0~\scriptsize($\pm$ 0.0) & \textbf{71.96}~\scriptsize($\pm$ \textbf{1.41}) & 48.65~\scriptsize($\pm$ 3.03)  & 0.0~\scriptsize($\pm$ 0.0)  \\

%WSN, $c=0.3$ & $\bsy \times$ & 75.98~\scriptsize($\pm$ 0.68) & 73.39~\scriptsize($\pm$ 1.53) & 0.0~\scriptsize($\pm$ 0.0) & 61.47~\scriptsize($\pm$ 0.30) & 49.72~\scriptsize($\pm$ 1.33) & 0.0~\scriptsize($\pm$ 0.0) & 70.92~\scriptsize($\pm$ 1.37) & 45.94~\scriptsize($\pm$ 2.35)  & 0.0~\scriptsize($\pm$ 0.0)  \\
WSN, $c=0.3$ & $\bsy \times$ & 75.98~\scriptsize($\pm$ 0.68) & 80.26~\scriptsize($\pm$ 1.53) & 0.0~\scriptsize($\pm$ 0.0) & 61.47~\scriptsize($\pm$ 0.30) & 63.47~\scriptsize($\pm$ 1.33) & 0.0~\scriptsize($\pm$ 0.0) & 70.92~\scriptsize($\pm$ 1.37) & 73.44~\scriptsize($\pm$ 2.35)  & 0.0~\scriptsize($\pm$ 0.0)  \\


%WSN, $c=0.5$ & $\bsy \times$ & 76.38~\scriptsize($\pm$ 0.34) & 92.26~\scriptsize($\pm$ 0.48) & 0.0~\scriptsize($\pm$ 0.0) & \textbf{61.79}~\scriptsize($\pm$ \textbf{0.23}) & 67.18~\scriptsize($\pm$ 1.58) & \textbf{0.0}~\scriptsize($\pm$ \textbf{0.0}) & 69.06~\scriptsize($\pm$ 0.82) & 64.53~\scriptsize($\pm$ 1.80)  & 0.0~\scriptsize($\pm$ 0.0)  \\
WSN, $c=0.5$ & $\bsy \times$ & \textbf{76.38}~\scriptsize($\pm$ \textbf{0.34}) & 99.13~\scriptsize($\pm$ 0.48) & 0.0~\scriptsize($\pm$ 0.0) & \textbf{61.79}~\scriptsize($\pm$ \textbf{0.23}) & 80.93~\scriptsize($\pm$ 1.58) & \textbf{0.0}~\scriptsize($\pm$ \textbf{0.0}) & 69.06~\scriptsize($\pm$ 0.82) & 92.03~\scriptsize($\pm$ 1.80)  & 0.0~\scriptsize($\pm$ 0.0)  \\


%WSN, $c=0.7$ & $\bsy \times$ & \textbf{76.88}~\scriptsize($\pm$ \textbf{0.51}) & 98.90~\scriptsize($\pm$ 0.16) & \textbf{0.0}~\scriptsize($\pm$ \textbf{0.0}) & 61.24~\scriptsize($\pm$ 0.16) & 83.65~\scriptsize($\pm$ 1.03) & 0.0~\scriptsize($\pm$ 0.0) & 67.18~\scriptsize($\pm$ 1.62) & 81.32~\scriptsize($\pm$ 1.32)  & 0.0~\scriptsize($\pm$ 0.0)  \\

%WSN, $c=0.7$ & $\bsy \times$ & \textbf{76.88}~\scriptsize($\pm$ \textbf{0.51}) & 105.77~\scriptsize($\pm$ 0.16) & \textbf{0.0}~\scriptsize($\pm$ \textbf{0.0}) 

% & 61.24~\scriptsize($\pm$ 0.16) & 97.40~\scriptsize($\pm$ 1.03) & 0.0~\scriptsize($\pm$ 0.0) 

% & 67.18~\scriptsize($\pm$ 1.62) & 108.82~\scriptsize($\pm$ 1.32)  & 0.0~\scriptsize($\pm$ 0.0)  \\

%WSN, $c=0.9$ & $\bsy \times$ & 75.04~\scriptsize($\pm$ 0.52) & 99.98~\scriptsize($\pm$ 0.01) & 0.0~\scriptsize($\pm$ 0.0) & 

%58.16~\scriptsize($\pm$ 0.56) & 96.78~\scriptsize($\pm$ 0.39) & 0.0~\scriptsize($\pm$ 0.0) 

%& 60.75~\scriptsize($\pm$ 1.02) & 94.25~\scriptsize($\pm$ 0.54)  & 0.0~\scriptsize($\pm$ 0.0)  \\

%WSN, $c=0.9$ & $\bsy \times$ & 75.04~\scriptsize($\pm$ 0.52) & 106.85~\scriptsize($\pm$ 0.01) & 0.0~\scriptsize($\pm$ 0.0) 

%& 58.16~\scriptsize($\pm$ 0.56) & 110.53~\scriptsize($\pm$ 0.39) & 0.0~\scriptsize($\pm$ 0.0) 

%& 60.75~\scriptsize($\pm$ 1.02) & 121.75~\scriptsize($\pm$ 0.54)  & 0.0~\scriptsize($\pm$ 0.0)  \\

\midrule

Multitask & $\bsy \times$ & 79.75~\scriptsize($\pm$ 0.38)$^\dagger$ & 100.0 & - & 61.00~\scriptsize($\pm$ 0.20)$^\dagger$ & 100.0  & - & 77.10~\scriptsize($\pm$ 1.06)$^\dagger$ & 100.0  & - \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:main_sota_table}
\end{center}
\end{table*}


==> materials/5_main_table_sota_full.tex <==
\begin{table*}[ht]
%\vspace{-0.1in}
\begin{center}
\caption{Performance comparisons of the proposed method and other state-of-the-art on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (ACC), average capacity (CAP), and average backward transfer (BWT) across $5$ independent runs with 5 seeds under the same experimental setup \cite{deng2021flattening}. The best results are highlighted in bold. Also, $\dagger$ $~$ and $\ast$ denotes results reported from \cite{deng2021flattening} and \cite{gupta2020maml} respectively.}

\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}}&\multicolumn{3}{c}{\textbf{CIFAR-100 Split}}&
\multicolumn{3}{c}{\textbf{CIFAR-100 Superclass}}&
\multicolumn{3}{c}{\textbf{TinyImageNet}} \\

\midrule
&ACC (\%)&CAP (\%)&BWT (\%)&
ACC (\%)&CAP (\%)&BWT (\%)&
ACC (\%)&CAP (\%)&BWT (\%) \\
\midrule


EWC \cite{Kirkpatrick2017} & 72.77~\scriptsize($\pm$ 0.45)$^\dagger$ & 100.0 & ~~-3.59~\scriptsize($\pm$ 0.55)$^\dagger$ & 50.26~\scriptsize($\pm$ 1.48)$^\dagger$ & 100.0  & ~~-7.87~\scriptsize($\pm$ 1.63)$^\dagger$ & - & - & -  \\

GEM \cite{Lopez-Paz2017} & 70.15~\scriptsize($\pm$ 0.34)$^\dagger$ & 100.0 & ~~-8.61~\scriptsize($\pm$ 0.42)$^\dagger$ & 50.35~\scriptsize($\pm$ 0.80)$^\dagger$ & 100.0  & ~~-9.50~\scriptsize($\pm$ 0.85)$^\dagger$ & 50.57~\scriptsize($\pm$ 0.61)$^\ast$ & 100.0 & -20.50~\scriptsize($\pm$ 0.10)$^\ast$  \\

ICARL \cite{rebuffi2017icarl} & 53.50~\scriptsize($\pm$ 0.81)$^\dagger$ & 100.0 & -20.44~\scriptsize($\pm$ 0.82)$^\dagger$ & 49.05~\scriptsize($\pm$ 0.51)$^\dagger$ & 100.0  & -11.24~\scriptsize($\pm$ 0.27)$^\dagger$ & 54.77~\scriptsize($\pm$ 0.32)$^\ast$ & 100.0 & ~~-3.93~\scriptsize($\pm$ 0.55)$^\ast$  \\

ER \cite{chaudhry2019continual} & 70.07~\scriptsize($\pm$ 0.35)$^\dagger$ & 100.0 & ~~-7.70~\scriptsize($\pm$ 0.59)$^\dagger$ & 51.64~\scriptsize($\pm$ 1.09)$^\dagger$ & 100.0  & ~~-7.86~\scriptsize($\pm$ 0.89)$^\dagger$ & 48.32~\scriptsize($\pm$ 1.51)$^\ast$ & 100.0 & -19.86~\scriptsize($\pm$ 0.70)$^\ast$  \\


La-MaML \cite{gupta2020maml} & 71.37~\scriptsize($\pm$ 0.67)$^\dagger$ & 100.0 & ~~-5.39~\scriptsize($\pm$ 0.53)$^\dagger$ & 54.44~\scriptsize($\pm$ 1.36)$^\dagger$ & 100.0  & ~~-6.65~\scriptsize($\pm$ 0.85)$^\dagger$ & 66.90~\scriptsize($\pm$ 1.65)$^\dagger$ & 100.0  & ~~-9.13~\scriptsize($\pm$ 0.90)$^\dagger$  \\
GPM \cite{Saha2021} & 73.18~\scriptsize($\pm$ 0.52)$^\dagger$ & 100.0 & ~~-1.17~\scriptsize($\pm$ 0.27)$^\dagger$ & 57.33~\scriptsize($\pm$ 0.37)$^\dagger$ & 100.0  & ~~-0.37~\scriptsize($\pm$ 0.12)$^\dagger$ & 67.39~\scriptsize($\pm$ 0.47)$^\dagger$ & 100.0  & ~~~\textbf{1.45~\scriptsize($\pm$ 0.22)}$^\dagger$  \\
FS-DGPM \cite{deng2021flattening} & 74.33~\scriptsize($\pm$ 0.31)$^\dagger$ & 100.0 & ~~-2.71~\scriptsize($\pm$ 0.17)$^\dagger$ & 58.81~\scriptsize($\pm$ 0.34)$^\dagger$  & 100.0  & ~~-2.97~\scriptsize($\pm$ 0.35)$^\dagger$ & 70.41~\scriptsize($\pm$ 1.30)$^\dagger$  & 100.0  & ~~-2.11~\scriptsize($\pm$ 0.84)$^\dagger$ \\
\midrule

PackNet \cite{mallya2018packnet} & 72.39~\scriptsize($\pm$ 0.37) & ~~96.38 \scriptsize($\pm$ 0.00) & \cellcolor{gg}\textbf{0.0} & 58.78~\scriptsize($\pm$ 0.52) & 126.65 \scriptsize($\pm$ 0.00) & \cellcolor{gg}\textbf{0.0} & 55.46~\scriptsize($\pm$ 1.22) & 188.67 \scriptsize($\pm$ 0.00) & \cellcolor{gg}\textbf{0.0} \\

SupSup \cite{wortsman2020supermasks} & 75.47~\scriptsize($\pm$ 0.30) & 129.00 \scriptsize($\pm$ 0.03) & \cellcolor{gg}\textbf{0.0} & 61.70~\scriptsize($\pm$ 0.31) & 162.49~\scriptsize($\pm$ 0.00) & \cellcolor{gg}\textbf{0.0} & 59.60~\scriptsize($\pm$ 1.05) & 214.52~\scriptsize($\pm$ 0.89) & \cellcolor{gg}\textbf{0.0} \\

\midrule

Hard-WSN, $c=0.03$ & 70.65~\scriptsize($\pm$ 0.36) & \textbf{18.56}~\scriptsize($\pm$ \textbf{0.25}) & \cellcolor{gg}\textbf{0.0} & 54.99~\scriptsize($\pm$ 0.71) & \textbf{22.30}~\scriptsize($\pm$ \textbf{0.22})  & \cellcolor{gg}\textbf{0.0} & 68.72~\scriptsize($\pm$ 1.63) & \textbf{37.19}~\scriptsize($\pm$ \textbf{0.21})  & \cellcolor{gg}\textbf{0.0}  \\

Hard-WSN, $c=0.05$ & 72.44~\scriptsize($\pm$ 0.27) & 25.09~\scriptsize($\pm$ 0.42) & \cellcolor{gg}\textbf{0.0} & 57.99~\scriptsize($\pm$ 1.34) & 27.37~\scriptsize($\pm$ 0.33)  & \cellcolor{gg}\textbf{0.0} & 71.22~\scriptsize($\pm$ 0.94) & 41.98~\scriptsize($\pm$ 0.52)  & \cellcolor{gg}\textbf{0.0}  \\

Hard-WSN, $c=0.1$ & 74.55~\scriptsize($\pm$ 0.47) & 39.87~\scriptsize($\pm$ 0.62) & \cellcolor{gg}\textbf{0.0} & 60.45~\scriptsize($\pm$ 0.37) & 38.55~\scriptsize($\pm$ 0.20)  & \cellcolor{gg}\textbf{0.0} & \textbf{71.96}~\scriptsize($\pm$ \textbf{1.41}) & 48.65~\scriptsize($\pm$ 3.03)  & \cellcolor{gg}\textbf{0.0}  \\

Hard-WSN, $c=0.3$ & 75.98~\scriptsize($\pm$ 0.68) & 80.26~\scriptsize($\pm$ 1.53) & \cellcolor{gg}\textbf{0.0} & 61.47~\scriptsize($\pm$ 0.30) & 63.47~\scriptsize($\pm$ 1.33) & \cellcolor{gg}\textbf{0.0} & 70.92~\scriptsize($\pm$ 1.37) & 73.44~\scriptsize($\pm$ 2.35)  & \cellcolor{gg}\textbf{0.0}  \\

Hard-WSN, $c=0.5$ & \textbf{76.38}~\scriptsize($\pm$ \textbf{0.34}) & 99.13~\scriptsize($\pm$ 0.48) & \cellcolor{gg}\textbf{0.0} & \textbf{61.79}~\scriptsize($\pm$ \textbf{0.23}) & 80.93~\scriptsize($\pm$ 1.58) & \cellcolor{gg}\textbf{0.0} & 69.06~\scriptsize($\pm$ 0.82) & 92.03~\scriptsize($\pm$ 1.80)  & \cellcolor{gg}\textbf{0.0}  \\

\midrule
Multitask & ~~79.75~\scriptsize($\pm$ 0.38)$^\dagger$ & 100.0 & - & ~~61.00~\scriptsize($\pm$ 0.20)$^\dagger$ & 100.0 & - & ~~77.10~\scriptsize($\pm$ 1.06)$^\dagger$ & 100.0 & - \\
\bottomrule
\end{tabular}}
%\end{adjustbox}
\label{tab:main_sota_full_table}
\end{center}
%\vspace{-0.2in}
\end{table*}

==> materials/5_per_layer_sparsity.tex <==
\begin{figure*}[ht]
    \centering
    \setlength{\tabcolsep}{-20pt}{%
    \begin{tabular}{ccc}
    \includegraphics[width=5.cm]{images/5_per_layer_sparsity_pmnist.pdf}&
    \includegraphics[width=5.cm]{images/5_per_layer_sparsity_cifar.pdf}&
    \includegraphics[width=5.cm]{images/5_per_layer_sparsity_5DATA.pdf} \\
    \multicolumn{3}{c}{(a) Layer Capacity over Increasing Number of Tasks} & 
    % \multicolumn{1}{c}{(b) SplitCIFAR100-AlexNet} &
    % \multicolumn{1}{c}{(c) Mixture-ResNet18}
    \\
    \end{tabular}}
    \caption{\footnotesize \textbf{\% used weights per layer vs \# of tasks seen}}
    \label{fig:per_layer_sparsity}
\end{figure*}

==> materials/5_same_network_different_data.tex <==
\begin{figure*}[ht]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ccc}
    \includegraphics[height=3.cm]{figures/p1.pdf}&
    \includegraphics[height=3.cm]{figures/p2.pdf}&
    \includegraphics[height=3.cm]{figures/p3.pdf} \\
    \multicolumn{1}{c}{(a) Lower Layer} & 
    \multicolumn{1}{c}{(b) Middle Layer} &
    \multicolumn{1}{c}{(c) Higher Layer}\\
    \end{tabular}}
    \caption{\footnotesize \textbf{Same Network Different Data - Catastrophic Forgetting as Property of Data}}
    \label{fig:cf_as_data_property}
\end{figure*}

==> materials/6_app_main_table.tex <==
\begin{table*}[t]
\tiny
\begin{center}
\caption{\small Performance comparison of the proposed method and other baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (Accuracy) and average forgetting (Forgetting) across $5$ independent runs. CF indicates that the method suffers from the catastrophic forgetting. The best results are highlighted in bold. Values with $\dagger$ $~$ denote reported performances from \cite{Saha2021}. PackNet~\cite{mallya2018packnet} is baseline.}

\begin{adjustbox}{width=1.0\textwidth}
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Method}}&\multicolumn{2}{c}{\textbf{Permuted MNIST}} & \multicolumn{2}{c}{\textbf{Split CIFAR-100}} & \multicolumn{2}{c}{\textbf{5 Datasets}} \\


\midrule
& CF & Accuracy & Capacity Used & Accuracy & Capacity Used & Accuracy & Capacity Used\\
\midrule
STL & $\bsy\times$ &
{\scriptsize 97.6} ($\pm$ 0.10) & {\scriptsize 1000.0} \%&
{\scriptsize 70.9} ($\pm$ 0.38) & {\scriptsize 1000.0} \%&
{\scriptsize 90.7} ($\pm$ 0.53) & {\scriptsize 500.0} \%\\
 \midrule
FINETUNE&  \checkmark &
{\scriptsize 62.5} ($\pm$ 2.96) & {\scriptsize 100.0} \%&
{\scriptsize 13.2} ($\pm$ 0.54) & {\scriptsize 100.0} \%&
{\scriptsize 36.8} ($\pm$ 2.25) & {\scriptsize 100.0} \%\\
HAT~\cite{Serra2018} &  \checkmark &
{\scriptsize -}  & {\scriptsize -} &
{\scriptsize 72.0} $\dagger$ & {\scriptsize 100.0} \%&
{\scriptsize 88.6} $\dagger$ & {\scriptsize 100.0} \%\\
% APD~\cite{Yoon2020}  & \checkmark &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%\\

AGS-CL~\cite{Jung2020} & \checkmark &
{\scriptsize 91.1} ($\pm$ 0.71) & {\scriptsize 100.0} \%&
{\scriptsize 49.6} ($\pm$ 1.89) & {\scriptsize 100.0} \%&
{\scriptsize -}  & -\\

GPM~\cite{Saha2021} & \checkmark &
% {\scriptsize 92.9} ($\pm$ 0.20) & {\scriptsize x.xx} \%&
{\scriptsize 93.9} $\dagger$ & {\scriptsize 100.0} \%&
{\scriptsize 72.5} $\dagger$ & {\scriptsize 100.0} \%&
{\scriptsize 91.3} $\dagger$ & {\scriptsize 100.0} \%\\
\cmidrule{1-8}
PackNet~\cite{mallya2018packnet}  & $\bsy\times$ &
%\textbf{{\scriptsize 95.9} ($\pm$ 0.05)} & {\scriptsize $~$ 96.8} \%& % 0.655 + 10*1/32
{\scriptsize 94.5} ($\pm$ 0.05) & {\scriptsize $~$ 72.1} \%& % 0.408 + 10*1/32
{\scriptsize 58.3} ($\pm$ 0.46) & {\scriptsize 131.2} \%& % 0.999 + 10*1/32
{\scriptsize 89.0} ($\pm$ 0.21) & {\scriptsize 115.4} \%\\ % 0.998 + 5 * 1/32
% LL-Ticket~\cite{longliveticket}  & $\bsy\times$ &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%\\
\cmidrule{1-8}
CST (Ours, SGD) $c=0.03$ & $\bsy\times$ &
{\scriptsize .} ($\pm$ 0.06) & \textbf{{\scriptsize $~$ 37.4}} \%&
{\scriptsize .} ($\pm$ 0.63) & \textbf{{\scriptsize $~$ 39.4}} \%&
{\scriptsize .} ($\pm$ 0.10) & \textbf{{\scriptsize $~$ 24.2}} \%\\
CST (Ours, SGD) $c=0.1$ & $\bsy\times$ &
{\scriptsize .} ($\pm$ 0.09) & {\scriptsize $~$ 46.3} \%&
{\scriptsize .} ($\pm$ 0.36) & {\scriptsize $~$ 56.2} \%&
{\scriptsize .} ($\pm$ 0.13) & {\scriptsize $~$ 39.9} \%\\
CST (Ours, SGD) $c=0.3$ & $\bsy\times$ &
{\scriptsize .} ($\pm$ 0.07) & {\scriptsize $~$ 68.3} \%& \textbf{{\scriptsize .} ($\pm$ 0.40)} & {\scriptsize $~$ .} \%& \textbf{{\scriptsize .} ($\pm$ 0.23)} & {\scriptsize $~$ 72.9} \%\\
CST (Ours, SGD) $c=0.5$ & $\bsy\times$ &
\textbf{{\scriptsize .} ($\pm$ 0.02)} & {\scriptsize $~$ 88.9} \%& {\scriptsize . ($\pm$ 0.92)} & {\scriptsize 111.0} \%& {\scriptsize .} ($\pm$ 0.13) & {\scriptsize $~$ 95.8} \%\\

\cmidrule{1-8}
CST (Ours, Adam) $c=0.03$ & $\bsy\times$ &
{\scriptsize 92.7} ($\pm$ 0.06) & \textbf{{\scriptsize $~$ 37.4}} \%&
{\scriptsize 65.6} ($\pm$ 0.63) & \textbf{{\scriptsize $~$ 39.4}} \%&
{\scriptsize 90.1} ($\pm$ 0.10) & \textbf{{\scriptsize $~$ 24.2}} \%\\
CST (Ours, Adam) $c=0.1$ & $\bsy\times$ &
{\scriptsize 93.9} ($\pm$ 0.09) & {\scriptsize $~$ 46.3} \%&
{\scriptsize 72.2} ($\pm$ 0.36) & {\scriptsize $~$ 56.2} \%&
{\scriptsize 91.3} ($\pm$ 0.13) & {\scriptsize $~$ 39.9} \%\\
CST (Ours, Adam) $c=0.3$ & $\bsy\times$ &
{\scriptsize 94.7} ($\pm$ 0.07) & {\scriptsize $~$ 68.3} \%& \textbf{{\scriptsize 73.5} ($\pm$ 0.40)} & {\scriptsize $~$ 97.4} \%& \textbf{{\scriptsize 91.7} ($\pm$ 0.23)} & {\scriptsize $~$ 72.9} \%\\
CST (Ours, Adam) $c=0.5$ & $\bsy\times$ &
\textbf{{\scriptsize 94.8} ($\pm$ 0.02)} & {\scriptsize $~$ 88.9} \%& {\scriptsize 72.5 ($\pm$ 0.92)} & {\scriptsize 111.0} \%& {\scriptsize 91.5} ($\pm$ 0.13) & {\scriptsize $~$ 95.8} \%\\
\cmidrule{1-8}
MTL &$\bsy\times$& {\scriptsize 96.7 $\dagger$} & {\scriptsize 100.0} \%& {\scriptsize 79.6 $\dagger$} & {\scriptsize 100.0} \%& {\scriptsize 91.5 $\dagger$} & {\scriptsize 100.0} \%\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:main_opt_table}
\end{center}
\end{table*}




==> materials/6_app_main_table_epoch.tex <==
\begin{table*}[t]
\tiny
\begin{center}
\caption{\small Performance comparison of the proposed method and other baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (Accuracy) and average forgetting (Forgetting) across $5$ independent runs. CF indicates that the method suffers from the catastrophic forgetting. The best results are highlighted in bold. Values with $\dagger$ $~$ denote reported performances from \cite{Saha2021}. PackNet~\cite{mallya2018packnet} is baseline.}

\begin{adjustbox}{width=1.0\textwidth}
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Method}}&\multicolumn{2}{c}{\textbf{Permuted MNIST}} & \multicolumn{2}{c}{\textbf{Split CIFAR-100}} & \multicolumn{2}{c}{\textbf{5 Datasets}} \\


\midrule
& CF & Accuracy & Capacity Used & Accuracy & Capacity Used & Accuracy & Capacity Used\\
\midrule
CST (Ours, epoch=10) $c=0.03$ & $\bsy\times$ &
{\scriptsize .} ($\pm$ 0.06) & \textbf{{\scriptsize $~$ 37.4}} \%&
{\scriptsize .} ($\pm$ 0.63) & \textbf{{\scriptsize $~$ 39.4}} \%&
{\scriptsize .} ($\pm$ 0.10) & \textbf{{\scriptsize $~$ 24.2}} \%\\
CST (Ours, Adam, epoch=10) $c=0.1$ & $\bsy\times$ &
{\scriptsize .} ($\pm$ 0.09) & {\scriptsize $~$ 46.3} \%&
{\scriptsize .} ($\pm$ 0.36) & {\scriptsize $~$ 56.2} \%&
{\scriptsize .} ($\pm$ 0.13) & {\scriptsize $~$ 39.9} \%\\
CST (Ours, Adam, epoch=10) $c=0.3$ & $\bsy\times$ &
{\scriptsize .} ($\pm$ 0.07) & {\scriptsize $~$ 68.3} \%& \textbf{{\scriptsize .} ($\pm$ 0.40)} & {\scriptsize $~$ .} \%& \textbf{{\scriptsize .} ($\pm$ 0.23)} & {\scriptsize $~$ 72.9} \%\\
CST (Ours, Adam, epoch=10) $c=0.5$ & $\bsy\times$ &
\textbf{{\scriptsize .} ($\pm$ 0.02)} & {\scriptsize $~$ 88.9} \%& {\scriptsize . ($\pm$ 0.92)} & {\scriptsize 111.0} \%& {\scriptsize .} ($\pm$ 0.13) & {\scriptsize $~$ 95.8} \%\\

\cmidrule{1-8}
CST (Ours, Adam, epoch=50) $c=0.03$ & $\bsy\times$ &
{\scriptsize 92.7} ($\pm$ 0.06) & \textbf{{\scriptsize $~$ 37.4}} \%&
{\scriptsize 65.6} ($\pm$ 0.63) & \textbf{{\scriptsize $~$ 39.4}} \%&
{\scriptsize 90.1} ($\pm$ 0.10) & \textbf{{\scriptsize $~$ 24.2}} \%\\
CST (Ours, Adam, epoch=50) $c=0.1$ & $\bsy\times$ &
{\scriptsize 93.9} ($\pm$ 0.09) & {\scriptsize $~$ 46.3} \%&
{\scriptsize 72.2} ($\pm$ 0.36) & {\scriptsize $~$ 56.2} \%&
{\scriptsize 91.3} ($\pm$ 0.13) & {\scriptsize $~$ 39.9} \%\\
CST (Ours, Adam, epoch=50) $c=0.3$ & $\bsy\times$ &
{\scriptsize 94.7} ($\pm$ 0.07) & {\scriptsize $~$ 68.3} \%& \textbf{{\scriptsize 73.5} ($\pm$ 0.40)} & {\scriptsize $~$ 97.4} \%& \textbf{{\scriptsize 91.7} ($\pm$ 0.23)} & {\scriptsize $~$ 72.9} \%\\
CST (Ours, Adam, epoch=50) $c=0.5$ & $\bsy\times$ &
\textbf{{\scriptsize 94.8} ($\pm$ 0.02)} & {\scriptsize $~$ 88.9} \%& {\scriptsize 72.5 ($\pm$ 0.92)} & {\scriptsize 111.0} \%& {\scriptsize 91.5} ($\pm$ 0.13) & {\scriptsize $~$ 95.8} \%\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:main_epoch_table}
\end{center}
\end{table*}




==> materials/6_app_main_table_new.tex <==
\begin{table*}[t]
\tiny
\begin{center}
\caption{\small (PMNIST, 5-Datasets, Omniglot Rotation) Performance comparison of the proposed method and other baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (Accuracy) and average forgetting (Forgetting) across $5$ independent runs. CF indicates that the method suffers from the catastrophic forgetting. The best results are highlighted in bold. Values with $\dagger$ $~$ denote reported performances from \cite{Saha2021}. PackNet~\cite{mallya2018packnet} is baseline.}

\begin{adjustbox}{width=1.0\textwidth}
\begin{tabular}{lccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Method}}&
% \multicolumn{3}{c}{\textbf{Permuted MNIST}} & 
\multicolumn{3}{c}{\textbf{Split CIFAR-100}} & 
\multicolumn{3}{c}{\textbf{Split CIFAR-100 Superclass}} \\ 
% \multicolumn{3}{c}{\textbf{5 Datasets}} & 
% \multicolumn{3}{c}{\textbf{Omniglot Rotation}} \\


\midrule
& CF & 
% ACC (\%) & CAP (\%) & BWT (\%) & 
ACC (\%) & CAP (\%) & BWT & 
% ACC (\%) & CAP (\%) & BWT (\%) & 
% ACC (\%) & CAP (\%) & BWT (\%) & 
ACC (\%) & CAP (\%) & BWT \\
\midrule
STL & $\bsy\times$ &
% {\scriptsize 97.6} ($\pm$ 0.10) & {\scriptsize 1000.0} \%& & 
% {\scriptsize 70.9} ($\pm$ 0.38) & {\scriptsize 1000.0} \%& & 
% {\scriptsize 90.7} ($\pm$ 0.53) & {\scriptsize 500.0} \% & &
% & & & 
% & & \\
% {\scriptsize 97.2} ($\pm$ 0.11) & {\scriptsize $~$ 1000} ($\pm$ 0.0) & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 73.9} ($\pm$ 0.44) & {\scriptsize $~$ 1000} ($\pm$ 0.0) & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 62.0} ($\pm$ 0.44) & {\scriptsize $~$ 2000} ($\pm$ 0.0) & {\scriptsize 0.0} ($\pm$ 0.0) \\
% {\scriptsize 93.4} ($\pm$ 0.12) & {\scriptsize $~$ 500} ($\pm$ 0.0) & {\scriptsize 0.0} ($\pm$ 0.0) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
 \midrule
FINETUNE&  \checkmark &
% {\scriptsize 62.5} ($\pm$ 2.96) & {\scriptsize 100.0} \%& &
% {\scriptsize 13.2} ($\pm$ 0.54) & {\scriptsize 100.0} \%& &
% {\scriptsize 36.8} ($\pm$ 2.25) & {\scriptsize 100.0} \%& & 
% & & & 
% & & \\
% {\scriptsize 30.4} ($\pm$ 2.82) & {\scriptsize $~$ 100} ($\pm$ 0.0) & {\scriptsize -73.5} ($\pm$ 3.14) &
{\scriptsize 57.1} ($\pm$ 1.1) & {\scriptsize $~$ 100.0} ($\pm$ 0.0) & {\scriptsize -0.22} ($\pm$ 0.01) &
{\scriptsize 37.3} ($\pm$ 1.6) & {\scriptsize $~$ 100.0} ($\pm$ 0.0) & {\scriptsize -0.28} ($\pm$ 0.02) \\
% {\scriptsize 56.9} ($\pm$ 0.91) & {\scriptsize $~$ 100} ($\pm$ 0.0) & {\scriptsize -45.4} ($\pm$ 1.16) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
HAT~\cite{Serra2018} &  \checkmark &
% {\scriptsize -}  & {\scriptsize -} & &
% {\scriptsize 72.0} $\dagger$ & {\scriptsize 100.0} \%& &
% {\scriptsize 88.6} $\dagger$ & {\scriptsize 100.0} \%& &
% & & &
% & & \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize 72.1} ($\pm$ 0.50) $\dagger$ & {\scriptsize $~$ 100.0} ($\pm$ 0.0) & {\scriptsize -0.00} ($\pm$ 0.00) $\dagger$ &
{\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
APD~\cite{Yoon2020}  & \checkmark &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize 56.8} ($\pm$ 0.33) $\dagger$ & {\scriptsize x.xx} \%& {\scriptsize -} ($\pm$ -) \\
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%& {\scriptsize -} ($\pm$ -) \\

AGS-CL~\cite{Jung2020} & \checkmark &
% {\scriptsize 91.1} ($\pm$ 0.71) & {\scriptsize 100.0} \%& &
% {\scriptsize 49.6} ($\pm$ 1.89) & {\scriptsize 100.0} \%& &
% {\scriptsize -}  & - & &
% & & & 
% & & \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
GPM~\cite{Saha2021} & \checkmark &
% {\scriptsize 92.9} ($\pm$ 0.20) & {\scriptsize x.xx} \%&
% {\scriptsize 93.9} $\dagger$ & {\scriptsize 100.0} \%& &
% {\scriptsize 72.5} $\dagger$ & {\scriptsize 100.0} \%& &
% {\scriptsize 91.3} $\dagger$ & {\scriptsize 100.0} \%& &
% & & & 
% & & \\
% {\scriptsize 93.9} ($\pm$ 0.16) $\dagger$ & \textbf{{\scriptsize $~$ 100} ($\pm$ 0.00)} & {\scriptsize -0.03} ($\pm$ 0.00) &
{\scriptsize 72.5} ($\pm$ 0.40) $\dagger$ & {\scriptsize $~$ 100.0} ($\pm$ 0.00) & {\scriptsize -0.00} ($\pm$ 0.00) &
{\scriptsize 57.7} ($\pm$ 0.37) $\dagger$ & {\scriptsize $~$ 100.0} ($\pm$ 0.00) & {\scriptsize -0.01} ($\pm$ 0.00) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
\midrule
PackNet~\cite{mallya2018packnet}  & $\bsy\times$ &
%\textbf{{\scriptsize 95.9} ($\pm$ 0.05)} & {\scriptsize $~$ 96.8} \%& % 0.655 + 10*1/32
% {\scriptsize 94.5} ($\pm$ 0.05) & {\scriptsize $~$ 72.1} \%& & % 0.408 + 10*1/32
% {\scriptsize 58.3} ($\pm$ 0.46) & {\scriptsize 131.2} \%& & % 0.999 + 10*1/32
% {\scriptsize 89.0} ($\pm$ 0.21) & {\scriptsize 115.4} \%& & % 0.998 + 5 * 1/32 
% & & & 
% & & \\ 
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize 72.5} ($\pm$ 0.21) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
% LL-Ticket~\cite{longliveticket}  & $\bsy\times$ &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%\\
\midrule
CST (Ours) $c=0.03$ & $\bsy\times$ & % need to add per-task sparsity
% {\scriptsize 95.0} ($\pm$ 0.11) & \textbf{{\scriptsize $~$ 13.1} ($\pm$ 0.06)} & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 71.0} ($\pm$ 0.56) & \textbf{{\scriptsize $~$ 11.7} ($\pm$ 0.25)} & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 62.5} ($\pm$ 0.40) & \textbf{{\scriptsize $~$ 10.4} ($\pm$ 0.24)} & {\scriptsize 0.0} ($\pm$ 0.0) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\

CST (Ours) $c=0.05$ & $\bsy\times$ & % need to add per-task sparsity
% {\scriptsize 95.6} ($\pm$ 0.15) & {\scriptsize $~$ 19.5} ($\pm$ 0.33) & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 72.4} ($\pm$ 0.44) & {\scriptsize $~$ 18.3} ($\pm$ 0.54) & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 63.1} ($\pm$ 0.16) & {\scriptsize $~$ 14.9} ($\pm$ 0.63) & {\scriptsize 0.0} ($\pm$ 0.0) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\

CST (Ours) $c=0.1$ & $\bsy\times$ & % need to add per-task sparsity
% {\scriptsize 96.2} ($\pm$ 0.10) & {\scriptsize $~$ 33.8} ($\pm$ 0.44) & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 74.7} ($\pm$ 0.33) & {\scriptsize $~$ 32.7} ($\pm$ 0.75) & {\scriptsize 0.0} ($\pm$ 0.0) &
\textbf{{\scriptsize 63.7} ($\pm$ 0.39)} & {\scriptsize $~$ 22.9} ($\pm$ 1.56) & \textbf{{\scriptsize 0.0} ($\pm$ 0.0)} \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\

CST (Ours) $c=0.3$ & $\bsy\times$ & % need to add per-task sparsity
% \textbf{{\scriptsize 96.5} ($\pm$ 0.06)} & {\scriptsize $~$ 70.2} ($\pm$ 0.50) & \textbf{{\scriptsize 0.0} ($\pm$ 0.0)} &
{\scriptsize 76.4} ($\pm$ 0.38) & {\scriptsize $~$ 73.1} ($\pm$ 0.81) & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 63.4} ($\pm$ 0.26) & {\scriptsize $~$ 38.2} ($\pm$ 0.74) & {\scriptsize 0.0} ($\pm$ 0.0) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\

CST (Ours) $c=0.5$ & $\bsy\times$ & % need to add per-task sparsity
% {\scriptsize 96.3} ($\pm$ 0.08) & {\scriptsize $~$ 90.9} ($\pm$ 0.31) & {\scriptsize 0.0} ($\pm$ 0.0) &
\textbf{{\scriptsize 76.5} ($\pm$ 0.39)} & {\scriptsize $~$ 92.2} ($\pm$ 0.75) & \textbf{{\scriptsize 0.0} ($\pm$ 0.0)} &
{\scriptsize 63.4} ($\pm$ 0.17) & {\scriptsize $~$ 57.0} ($\pm$ 0.63) & {\scriptsize 0.0} ($\pm$ 0.0) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\

\midrule
MTL &$\bsy\times$& 
% {\scriptsize 96.7 $\dagger$} & {\scriptsize 100.0} \% & {\scriptsize -} & 
{\scriptsize 79.6 $\dagger$} & {\scriptsize 100} & {\scriptsize -} & 
% {\scriptsize 91.5 $\dagger$} & {\scriptsize 100.0} \% & {\scriptsize -} \\
{\scriptsize 61.0 $\dagger$} & {\scriptsize 100} & {\scriptsize -} \\ 
% {\scriptsize -} & {\scriptsize -} \% & {\scriptsize -} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:main_table}
\end{center}
\end{table*}




==> materials/6_app_plots_acc_vs_cap.tex <==
\begin{figure}[ht]
    \centering
    \vspace{-0.1in}
    \renewcommand{\arraystretch}{1}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    \includegraphics[width=.5\columnwidth]{images/5_acc_vs_cap_pmnist_new_w_dots_no_title.pdf} &
    \includegraphics[width=.5\columnwidth]{images/5_acc_vs_cap_omniglot_rotation_new_wo_packnet_w_dots_no_title.pdf} \\
    % \vspace{-0.06in}
    \small (a) PMNIST - MLP & \small (b) Omniglot Rotation - LeNet \\
    % \vspace{-0.06in}
    \end{tabular}}
    % \vspace{-0.15in}
    \caption{\footnotesize \textbf{Accuracy over Total Capacity Usage}: WSN achieves best performance under Accuracy-Capacity trade-off in PMNIST and Omniglot Rotation datasets - It can be seen that WSN's accuracy is higher than other competing baselines, especially PackNet, while utilizing less total capacity.}
    \label{fig:acc_vs_cap_appendix}
    % \vspace{-0.1in}
\end{figure}

==> materials/7_main_confusion_omniglot.tex <==
\begin{figure}[ht]
    \centering
    %\setlength{\tabcolsep}{-9pt}{%
    %\begin{tabular}{cccc}
    %\includegraphics[height=3.45cm]{images/corr_binary_Omniglot Rotation_seed_5_capacity_5.pdf} &~\;\;
    %\includegraphics[height=3.45cm]{images/corr_binary_Omniglot Rotation_seed_1_capacity_10.pdf} &~\;\; 
    %\includegraphics[height=3.45cm]{images/corr_binary_Omniglot Rotation_seed_3_capacity_30.pdf} &~\;\;
    %\includegraphics[height=3.45cm]{images/corr_binary_Omniglot Rotation_seed_9_capacity_50.pdf} \\ 
    %\small (a) $c=0.05$ & \small (b) $c=0.1$ & 
    %\small (c) $c=0.3$ & \small (d) $c=0.5$ \\
    %\end{tabular}
    %}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    % we prepare the figure 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_Omniglot Rotation_seed_5_capacity_5.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_Omniglot Rotation_seed_1_capacity_10.pdf} \\
    \small (a) $c=5\%$ & \small (b) $c=10\%$ \\
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_Omniglot Rotation_seed_3_capacity_30.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_Omniglot Rotation_seed_9_capacity_50.pdf} \\
    \small (c) $c=30\%$ & \small (d) $c=50\%$
    \end{tabular}}
    
    \caption{\footnotesize \textbf{Average Binary Map Correlation} on Sequence of Omniglot Rotation Experiments: the binary maps get overlapped with prior ones as the number of tasks increases..}
    \label{fig:main_omniglot_conf}
    %\vspace{12cm}
\end{figure}

==> rebuttals/IFSL_5way_5shot.tex <==
\begin{table}[t]
\captionsetup{font={color=blue}}
\vspace{-0.2in}
\begin{center}
\caption{\small Classification accuracy on CIFAR-100 for 5-way 5-shot incremental learning, compared with the SOTA \textbf{[1]}.}
%\vspace{-0.1in}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{9}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\textbf{cRT}}} \\ 
\cline{2-10}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &  \\
\midrule
cRT & 65.18 & 63.89 & 60.20 & 57.23 & 53.71 & 50.39 & 48.77 & 47.29 & 45.28 & - \\
%Joint-training & 65.18 & 61.45 & 57.36 & 53.68 & 50.84 & 47.33 & 44.79 & 42.62 & 40.08 & -5.20 \\
%Baseline & 65.18 & 61.67 & 58.61 & 55.11 & 51.86 & 49.43 & 47.60 & 45.64 & 43.83 & -1.45 \\
\midrule
%iCaRL [40]∗ & 66.52 & 57.26 & 54.27 & 50.62 & 47.33 & 44.99 & 43.14 & 41.16 & 39.49 & -5.79 \\
%Rebalance [20]∗ & 66.66 & 61.42 & 57.29 & 53.02 & 48.85 & 45.68 & 43.06 & 40.56 & 38.35 & -6.93 \\
%FSLL [34]∗ & 65.18 & 56.24 & 54.55 & 51.61 & 49.11 & 47.27 & 45.35 & 43.95 & 42.22 & -3.08 \\
%iCaRL [40] & 64.10 & 53.28 & 41.69 & 34.13 & 27.93 & 25.06 & 20.41 & 15.48 & 13.73 & -31.55 \\
%Rebalance [20] & 64.10 & 53.05 & 43.96 & 36.97 & 31.61 & 26.73 & 21.23 & 16.78 & 13.54 & -31.74 \\
%TOPIC [47] & 64.10 & 55.88 & 47.07 & 45.16 & 40.11 & 36.38 & 33.96 & 31.55 & 29.37 & -15.91 \\
%FSLL & 64.10 & 55.85 & 51.71 & 48.59 & 45.34 & 43.25 & 41.52 & 39.81 & 38.16 & -7.12 \\
FSLL+SS & 66.76 & 55.52 & 52.20 & 49.17 & 46.23 & 44.64 & 43.07 & 41.20 & 39.57 & -5.71 \\
F2M (SOTA) & 64.71 & 62.05 & 59.01 & 55.58 & 52.55 & 49.96 & 48.08 & 46.28 & 44.67 & -0.61 \\
\midrule 
\textcolor{red}{WSN}, $c=0.502$ & \textbf{72.63} & \textbf{68.36} & \textbf{64.59} & \textbf{60.77} & \textbf{57.57} & \textbf{54.81} & \textbf{52.73} & \textbf{50.47} & \textbf{48.13} & \textbf{+2.85} \\ 
\bottomrule
\end{tabular}}
\label{tab:cifar100_5way_5shot}
\end{center}
\vspace{-0.35in}
\end{table}

==> rebuttals/init_reinit.tex <==
\begin{figure}[ht]
    \centering
    %\vspace{-0.05in}
    \setlength{\tabcolsep}{-7pt}{%
    \begin{tabular}{cc}
    \includegraphics[height=2.96cm,trim={0.3cm 0.1cm 0.1cm 0.1cm},clip]{rebuttals/images/_reinit_avg_all_capa_csnb_tiny_data.pdf} &\;\; 
    \includegraphics[height=2.96cm,trim={0.1cm 0.1cm 0.1cm 0.1cm},clip]{rebuttals/images/2_avg_all_capa_csnb_tiny_data.pdf} \\
    \small (a) re-initialized for each task & \small (b) initialized only ones
    \end{tabular}}
    \vspace{-0.1in}
    \caption{\textbf{WSN's Comparisons of Capacities} on TinyImageNet Dataset: (a) re-initialized weight score per task and (b) initialized weight score only once before training task 1.}
    \label{fig:reinit_tiny}
    \vspace{-0.05in}
\end{figure}

==> rebuttals/table2_reinit.tex <==
\begin{table}[ht]
%\small
\begin{center}
%\captionsetup{labelfont{color=blue}}
\caption{Performance comparisons of Re-initialized WSN and Initialized ones with $c = 50\%$ on the three benchmark datasets.}
%\vspace{-0.05in}

\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}}&\multicolumn{2}{c}{\textbf{CIFAR-100 Split}}&
\multicolumn{2}{c}{\textbf{CIFAR-100 Superclass}}&
\multicolumn{2}{c}{\textbf{TinyImageNet}} \\

\midrule
WSN &ACC (\%) & CAP (\%) & ACC (\%) & CAP (\%) & ACC (\%) & CAP (\%) \\
\midrule

Re-init. & 75.68~\scriptsize($\pm$ 0.42) & 104.47\scriptsize($\pm$ 0.00) & 61.72~\scriptsize($\pm$ 0.29) & 113.74~\scriptsize($\pm$ 0.00) & 61.13~\scriptsize($\pm$ 1.13) & 127.49~\scriptsize($\pm$ 0.00)  \\

Init. & \textbf{76.38}~\scriptsize($\pm$ \textbf{0.34}) & \textbf{99.13}~\scriptsize($\pm$ \textbf{0.48}) & \textbf{61.79}~\scriptsize($\pm$ \textbf{0.23}) & \textbf{80.93}~\scriptsize($\pm$ \textbf{1.58}) & \textbf{69.06}~\scriptsize($\pm$ \textbf{0.82}) & \textbf{92.03}~\scriptsize($\pm$ \textbf{1.80})  \\

\bottomrule
\end{tabular}}
%\end{adjustbox}
\label{tab:table2_reinit}
\end{center}
\vspace{-0.1in}
\end{table}

==> soft-materials/2_intro/3_concept.tex <==
\begin{figure*}
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    %\setlength{\tabcolsep}{-0pt}{%
    \begin{tabular}{ccc}
    \includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/smooth_subnet/1_concept_smooth_subnetwork0.pdf} &
    \includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/smooth_subnet/1_concept_smooth_subnetwork1.pdf} &
    \includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/smooth_subnet/1_concept_smooth_subnetwork2.pdf} \\
    
    \makecell{\small{(a) Dense \textcolor{orange}{Initialization}}} &
    \makecell{\small{(b)  \textcolor{blue}{Training} of SoftNet}} &
    \makecell{\small{(c) \textcolor{red}{Update} of SoftNet}}\\
    \end{tabular}
    %\end{adjustbox}
    % \vspace{-0.05in}
    \caption{\small \textbf{Incremental Soft-Subnetwork (SoftNet):} (a) Dense Neural Network is randomly initialized for the base session (S-1) training (b) SoftNet is trained by major subnetwork $\bm{m}_{\textcolor{black}{major}}=1$ (\textcolor{blue}{thick solid line}) and minor $\bm{m}_{\textcolor{black}{minor}} \sim U(0,1)$, and (c) SoftNet updates only a few minor weights (\textcolor{red}{thin solid line}) for new sessions (S).}
    \label{fig:concept_softnet}
\end{figure*}

==> soft-materials/6_exper/3_concept_tsnes.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    \setlength{\tabcolsep}{-0pt}{%
    \begin{tabular}{ccc}
    \includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.1cm},clip]{images/tsne/sess0_task_id1} \\
    \includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.1cm},clip]{images/tsne/sess0_task_id2} \\
    \includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.1cm},clip]{images/tsne/sess0_task_id3} \\
    \includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.1cm},clip]{images/tsne/sess0_task_id4} \\
    %\includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.06cm},clip]{images/1_concept_biased_transfer.pdf} &
    %\includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.06cm},clip]{images/1_concept_slective_re_used.pdf} &
    %\includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.06cm},clip]{images/1_concept_wsns.pdf} \\ 
    
    %\makecell{\small (a) Fixed Backbone \\ \small Network} &
    %\makecell{\small (b) Biased \small Transfer} &
    %\makecell{\small (c) Selective Reuse Expansion \\ \small beyond Full Network} &
    %\makecell{\small (d) Selective Reuse Expansion \\ \small within Network (Our WSN)} \\
    \end{tabular}
    }
    \caption{\small \textbf{Subnetworks with few weights, $0.002$}}
    \label{fig:concept_comparison}
    \vspace{-0.1in}
\end{figure*}

==> soft-materials/6_exper/5_main_cifar100_hardnet.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy on CIFAR-100 for 5-way 5-shot FSCIL with varying capasity $c$ and $c_l=1.002$.}

\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{9}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\makecell{\textbf{The gap} \\ \textbf{with cRT}}}} \\ 
\cline{2-10}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &  \\
\midrule
cRT & 65.18 & 63.89 & 60.20 & 57.23 & 53.71 & 50.39 & 48.77 & 47.29 & 45.28 & - \\
\midrule
% ---- varying capasity from 0.5 to 0.99 --------
HardNet, $c=0.80$ ,$c_l=0.002$   
& 72.22	& 67.99 & 64.32 & 60.58 & 57.45 & 54.74 & 52.92 & 50.89 & 48.65 & +3.37
\\
HardNet, $c=0.90$ ,$c_l=0.002$
& 72.78 & 68.56 & 64.93 & 61.33 & 58.2 & 55.56 & 53.59 & 51.47 & 49.26 & +3.98
\\
HardNet, $c=0.93$ ,$c_l=0.002$  
& 72.57 & 68.31 & 64.77 & 61.09 & 57.91 & 55.32 & 53.50 & 51.38 & 49.18 & +3.9
\\
HardNet, $c=\bm{0.95}$ ,$c_l=0.002$  
& \textbf{72.85} & \textbf{68.67} & \textbf{65.08} & \textbf{61.33} & \textbf{58.20} & \textbf{55.51} & \textbf{53.52} & \textbf{51.61} & \textbf{49.33} & +\textbf{4.05}
\\
HardNet, $c=0.97$ ,$c_l=0.002$  
& 72.60 & 68.51 & 64.79 & 60.99 & 57.9 & 55.08 & 53.33 & 51.31 & 49.21 & +3.93
\\
HardNet, $c=0.99$ ,$c_l=0.002$  
& 72.75 & 68.05 & 64.39 & 60.71 & 57.52 & 54.90 & 53.09 & 51.04 & 48.92 & +3.64
\\
\midrule
% ---- varying new capasity from c_l = 0.002 to 0.5 --------
HardNet, $c=0.95$, $c_l=0.002$  
& 72.85 & 68.67 & 65.08 & 61.33 & 58.20 & 55.51 & 53.52 & 51.61 & 49.33 & +4.05
\\
HardNet, $c=0.95$, $c_l=0.1$  
& \textbf{72.85} & \textbf{68.78} & \textbf{65.19}	& \textbf{61.44} & \textbf{58.29}	& \textbf{55.60}	& \textbf{53.61} & \textbf{51.70} & \textbf{49.40} & +\textbf{4.12}
\\
HardNet, $c=0.95$, $c_l=0.3$ 
& 72.85 & 68.51 & 64.98 & 61.24 & 58.13 & 55.42 & 53.44 & 51.54 & 49.26 &+3.98
\\
HardNet, $c=0.95$, $c_l=0.5$  
& 72.85	& 68.52 & 65.00	& 61.25 & 58.13 & 55.41 & 53.41 & 51.51 & 49.23 & +3.95
\\
HardNet, $c=0.95$, $c_l=0.7$  
& 72.85 & 68.63 & 65.10 & 61.33 & 58.19 & 55.50	& 53.49 & 51.59 & 49.31	& +4.03
\\
HardNet, $c=0.95$, $c_l=0.9$  
& 72.85 & 68.62 & 65.07 & 61.30 & 58.17 & 55.46 & 53.43 & 51.51 & 49.23 & +3.95
\\
\bottomrule
\end{tabular}}
\label{tab:cifar100_5way_5shot_hardnet}
\end{center}
\end{table*}

==> soft-materials/6_exper/5_main_cifar100_hardnet_baseline.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy of ResNet18 v.s. ResNet20 on CIFAR-100 for 5-way 5-shot FSCIL with varying capacity $c$. \underbar{Underbar} denotes the comparable results with baseline. $^\ast$ denotes results reported from \cite{shi2021overcoming}.}

\resizebox{0.92\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{9}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\makecell{\textbf{The gap} \\ \textbf{with cRT}}}} \\ 
\cline{2-10}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &  \\
\midrule
ResNet18, cRT \cite{shi2021overcoming} & 65.18 & 63.89 & 60.20 & 57.23 & 53.71 & 50.39 & 48.77 & 47.29 & 45.28 & - \\
ResNet18, Joint-training \cite{shi2021overcoming} & 65.18 & 61.45 & 57.36 & 53.68 & 50.84 & 47.33 & 44.79 & 42.62 & 40.08 & -5.20 \\
ResNet18, Baseline \cite{shi2021overcoming} & 65.18 & 61.67 & 58.61 & 55.11 & 51.86 & 49.43 & 47.60 & 45.64 & 43.83 & -1.45 \\
\midrule
%iCaRL~\cite{rebuffi2017icarl}$^\ast$ & 66.52 & 57.26 & 54.27 & 50.62 & 47.33 & 44.99 & 43.14 & 41.16 & 39.49 & -5.79 \\
%Rebalance~\cite{hou2019learning}$^\ast$ & 66.66 & 61.42 & 57.29 & 53.02 & 48.85 & 45.68 & 43.06 & 40.56 & 38.35 & -6.93 \\
%FSLL~\cite{mazumder2021few}$^\ast$ & 65.18 & 56.24 & 54.55 & 51.61 & 49.11 & 47.27 & 45.35 & 43.95 & 42.22 & -3.08 \\
%iCaRL \cite{rebuffi2017icarl} & 64.10 & 53.28 & 41.69 & 34.13 & 27.93 & 25.06 & 20.41 & 15.48 & 13.73 & -31.55 \\
%Rebalance \cite{hou2019learning} & 64.10 & 53.05 & 43.96 & 36.97 & 31.61 & 26.73 & 21.23 & 16.78 & 13.54 & -31.74 \\
%TOPIC~\cite{cheraghian2021semantic} & 64.10 & 55.88 & 47.07 & 45.16 & 40.11 & 36.38 & 33.96 & 31.55 & 29.37 & -15.91 \\
%F2M~\cite{shi2021overcoming} & 64.71 & 62.05 & 59.01 & 55.58 & 52.55 & 49.96 & 48.08 & 46.28 & 44.67 & -0.61 \\
%\midrule
%FSLL \cite{mazumder2021few} & 64.10 & 55.85 & 51.71 & 48.59 & 45.34 & 43.25 & 41.52 & 39.81 & 38.16 & -7.12 \\
ResNet18, HardNet, $c=10\%$   
& 28.97	& 27.71 & 26.08 & 24.68	& 23.34 & 22.02 & 21.12 & 20.48 & 19.50 & -25.78 \\
ResNet18, HardNet, $c=20\%$   
& 37.42	& 35.29 & 33.22 & 31.32 & 29.51 & 27.80 & 26.54 & 25.28 & 24.16 & -21.12 \\
ResNet18, HardNet, $c=30\%$   
& 55.47	& 52.37 & 49.38 & 46.53 & 43.88 & 41.50 & 39.58 & 37.82 & 36.06	& -9.22 \\
ResNet18, HardNet, $c=40\%$   
& 57.52	& 53.85 & 50.62 & 47.74 & 44.90 & 42.64 & 40.76 & 38.95 & 37.07	& -8.21 \\
ResNet18, HardNet, $c=50\%$   
& \underbar{64.80}	& \underbar{60.77} & \underbar{56.95} & \underbar{53.53} & \underbar{50.40} & \underbar{47.82} & \underbar{45.93} & \underbar{43.95} & \underbar{41.91}	& -\underbar{3.37} \\
ResNet18, HardNet, $c=60\%$   
& 66.72	& 62.21 & 58.14 & 54.60 & 51.47 & 48.86 & 46.67 & 44.67 & 42.66	& -2.62 \\
ResNet18, HardNet, $c=70\%$   
& 68.27 & 63.52 & 59.45 & 55.89 & 52.91 & 50.30 & 48.27 & 46.25 & 44.22	& -1.06 \\
ResNet18, HardNet, $c=80\%$   
& 69.65	& 64.60 & 60.59 & 56.93 & 53.60 & 50.80 & 48.69 & 46.69 & 44.63	& -0.65 \\
ResNet18, HardNet, $c=90\%$ 
& 70.85 & 65.84 & 61.59 & 57.92 & 54.65 & 51.90 & 49.79 & 47.66 & 45.47 & +0.19 \\
ResNet18, HardNet, $c=93\%$   
& 71.22	& 66.20 & 62.00 & 58.34 & 55.04 & 52.34 & 50.22 & 48.07 & 46.04 & +0.76 \\
ResNet18, HardNet, $c=95\%$   
& 71.73	& 66.31 & 62.17 & 58.44 & 54.98	& 52.20 & 50.17 & 47.97 & 45.87	& +0.59 \\ 
ResNet18, HardNet, $c=97\%$   
& 71.85	& 66.48 & 62.29	& 58.62 & 55.36 & 52.55 & 50.60 & 48.43 & 46.22	& +0.94 \\
ResNet18, HardNet, $c=99\%$  
&71.95 & 66.83 & 62.75 & 59.09 & 55.92 & 53.03 & 50.78 & 48.52 & 46.31 & +1.03 \\
\midrule
% ---- layer4  --------
ResNet18, SoftNet, ~~$c=10\%$   
& 60.77	& 57.02 & 53.62 & 50.51 & 47.67 & 45.14 & 43.32 & 41.6 & 39.58 & -5.7 \\
ResNet18, SoftNet, ~~$c=20\%$   
& 64.67	& 60.69 & 57.15 & 53.77 & 50.76 & 48.28 & 46.24 & 44.23 & 42.31	& -2.97 \\
ResNet18, SoftNet, ~~$c=30\%$   
& 67.00 & 62.18 & 58.22 & 54.69 & 51.82 & 49.12 & 47.13 & 44.98 & 42.44 & -2.84 \\
ResNet18, SoftNet, ~~$c=40\%$   
& 67.50 & 63.11 & 59.29 & 55.61 & 52.53 & 49.85 & 47.85 & 45.84 & 43.85 & -1.43 \\
ResNet18, SoftNet, ~~$c=50\%$   
& 69.20 & 64.18 & 60.01 & 56.43 & 53.11 & 50.62 & 48.60 & 46.51 & 44.61 & -0.67 \\
ResNet18, SoftNet, ~~$c=60\%$ 
& 69.15	& 63.68 & 59.54 & 56.05 & 52.72 & 50.10 & 48.20 & 46.18 & 44.15 & -1.13 \\
ResNet18, SoftNet, ~~$c=70\%$ 
& 70.92 & 65.16 & 61.00 & 57.25 & 54.09 & 51.37 & 49.29 & 47.03 & 44.90 & -0.38 \\
ResNet18, SoftNet, ~~$c=80\%$ 
& 70.38 & 65.04 & 60.94 & 57.26 & 54.13 & 51.58 & 49.52 & 47.36 & 45.16 & -0.12 \\
ResNet18, SoftNet, ~~$c=90\%$ 
& 72.25	& 66.82 & 62.63 & 58.98 & 55.64 & 52.77 & 50.71 & 48.42 & 46.15 & +0.87 \\
ResNet18, SoftNet, ~~$c=93\%$ 
& 71.38	& 65.93 & 61.89 & 58.20 & 54.87 & 51.83 & 49.82 & 47.57 & 45.47 & +0.19 \\
ResNet18, SoftNet, ~~$c=95\%$ 
& 72.23 & 66.94 & 62.56 & 58.84 & 55.65 & 52.74 & 50.61 & 48.47 & 46.27 & +0.99 \\
ResNet18, SoftNet, ~~$c=97\%$ 
& 70.88	& 65.72 & 61.38 & 57.88 & 54.63 & 51.82 & 49.57 & 47.30 & 45.19	& -0.09 \\
ResNet18, SoftNet, ~~$c=99\%$ 
& \textbf{72.62} & \textbf{67.31} & \textbf{63.05} & \textbf{59.39}	& \textbf{56.00} & \textbf{53.23} & \textbf{51.06} & \textbf{48.83} & \textbf{46.63} & +\textbf{1.35}\\
\bottomrule


% ---- euc distance measurements without training  --------
ResNet20, HardNet, ~$c=10\%$   
& 53.50  & 50.52 & 47.79 & 45.11 & 42.57 & 40.38 & 38.88 & 37.43 & 35.69 & -9.59 \\

ResNet20, HardNet, ~$c=20\%$   
& 61.83 & 58.24 & 55.17 & 51.92 & 49.07 & 46.68 & 45.02 & 43.31 & 41.40 & -3.88 \\

ResNet20, HardNet, ~$c=30\%$   
& \underbar{66.68} & \underbar{62.81} &  \underbar{59.54} & \underbar{56.12} & \underbar{53.21} & \underbar{50.52} & \underbar{48.85} & \underbar{46.93} & \underbar{44.84} & -\underbar{0.44} \\
ResNet20, HardNet, ~$c=40\%$   
& 68.31 & 64.17 & 60.72 & 57.19 & 54.26 & 51.79 & 50.13 & 48.01 & 45.93 & +0.65 \\

ResNet20, HardNet, ~$c=50\%$   
& 70.73 & 66.56 & 63.10 & 59.59 & 56.58 & 53.87 & 51.86 & 49.72 & 47.46 & +2.18 \\

ResNet20, HardNet, ~$c=60\%$   
& 71.90	& 67.64 & 63.84 & 60.22 & 57.06 & 54.30 & 52.53 & 50.53 & 48.34 & +3.06 \\

ResNet20, HardNet, ~$c=70\%$   
& 71.41	& 67.44 & 63.76 & 60.02 & 56.84 & 54.14 & 52.54 & 50.42 & 48.24 & +2.96 \\

ResNet20, HardNet, ~$c=80\%$   
& 71.97 & 67.65 & 63.93 & 60.14 & 57.12 & 54.44 & 52.72 &50.67	& 48.43 & +3.15 \\

ResNet20, HardNet, ~$c=90\%$ 
& 71.82 & 67.73 & 64.21 & 60.44 & 57.44 & 54.93 & 53.14 & 51.03	& 48.86 & +3.58 \\

ResNet20, HardNet, ~$c=93\%$   
& 72.28 & 67.99 & 64.48 & 60.83 & 57.64 & 55.16 & 53.27 & 51.11	& 48.93 & +3.65 \\
ResNet20, HardNet, ~$c=95\%$   
& 72.13 & 68.14 & 64.50 & 60.74 & 57.68 & 55.12 & 53.17 & 51.23	& 48.97 & +3.69 \\ 
ResNet20, HardNet, ~$c=97\%$   
& 71.90	& 67.81 & 64.11 & 60.24 & 57.14 & 54.41 & 52.74 & 50.71 & 48.67 & +3.39 \\
\midrule
% ---- layer3  --------
ResNet20, SoftNet, ~~$c=10\%$   
& 53.13 & 49.73 & 46.85 & 44.01 & 41.54 & 39.45 & 37.84 & 36.30 & 34.62 & -10.66 \\
ResNet20, SoftNet, ~~$c=20\%$   
& 60.15 & 56.25	& 53.26 & 50.16 & 47.46 & 45.23 & 43.75 & 41.84 & 39.90 & -5.38 \\
ResNet20, SoftNet, ~~$c=30\%$   
& 64.65	& 59.99 & 56.65 & 53.45 & 50.42 & 48.02 & 46.48 & 44.61 & 42.43 & -2.85 \\
ResNet20, SoftNet, ~~$c=40\%$   
& 66.77	& 62.55 & 59.35 & 55.63 & 52.70 & 50.21 & 48.54 & 46.60 & 44.50 & -0.78 \\
ResNet20, SoftNet, ~~$c=50\%$   
& 68.20 & 64.21 & 60.78 & 57.15 & 54.20 & 51.53 & 49.84 & 47.92 & 45.84 & +0.56 \\
ResNet20, SoftNet, ~~$c=60\%$ 
& 68.63	& 64.76 & 61.00 & 57.53 & 54.56 & 52.11 & 50.34 & 48.41 & 46.30 & +1.02 \\
ResNet20, SoftNet, ~~$c=70\%$ 
& 70.38	& 66.16 & 62.63 & 58.93 & 55.81 & 53.11 & 51.38 & 49.29 & 47.08 & +1.80 \\
ResNet20, SoftNet, ~~$c=80\%$ 
& 70.87	& 66.47 & 62.85 & 59.28 & 56.27 & 53.84 & 52.01 & 50.16 & 48.01 & +2.73 \\
ResNet20, SoftNet, ~~$c=90\%$ 
& 72.63	& \textbf{68.60} & \textbf{64.96} & \textbf{61.25} & \textbf{57.98} & \textbf{55.32} & \textbf{53.48} & \textbf{51.46} & \textbf{49.20} & +\textbf{3.92} \\
ResNet20, SoftNet, ~~$c=93\%$ 
& 72.53 & 68.45 & 64.59 & 60.80 & 57.48 & 54.91 & 53.19 & 51.03 & 48.83 & +3.55 \\
ResNet20, SoftNet, ~~$c=95\%$ 
& 72.58 & 68.30 & 64.57 & 60.83 & 57.67 & 54.86 & 53.11 & 51.21 & 49.06 & +3.78 \\
ResNet20, SoftNet, ~~$c=97\%$ 
& \textbf{72.80} & 68.46 & 64.61 & 60.90 & 57.63 & 54.95 & 53.26 & 51.12 & 48.95 & +3.67 \\
ResNet20, SoftNet, ~~$c=99\%$ 
& 71.78	& 67.79 & 63.86 & 60.07 & 57.05 & 54.32 & 52.34 & 50.28 & 48.11 & +2.83 \\
\bottomrule

\end{tabular}}
\label{tab:cifar100_5way_5shot_hardnet_resnet20}
\end{center}
\end{table*}

==> soft-materials/6_exper/5_main_cifar100_resnet18_5way_5shot.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy of ResNet18 on CIFAR-100 for 5-way 5-shot incremental learning. \underbar{Underbar} denotes the comparable results with baseline. $^\ast$ denotes the results reported from \cite{shi2021overcoming}.}

\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{9}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\makecell{\textbf{The gap} \\ \textbf{with cRT}}}} \\ 
\cline{2-10}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &  \\
\midrule
cRT~\cite{shi2021overcoming} & 65.18 & 63.89 & 60.20 & 57.23 & 53.71 & 50.39 & 48.77 & 47.29 & 45.28 & - \\
Joint-training~\cite{shi2021overcoming} & 65.18 & 61.45 & 57.36 & 53.68 & 50.84 & 47.33 & 44.79 & 42.62 & 40.08 & -5.20 \\
Baseline~\cite{shi2021overcoming} & 65.18 & 61.67 & 58.61 & 55.11 & 51.86 & 49.43 & 47.60 & 45.64 & 43.83 & -1.45 \\
\midrule
iCaRL~\cite{rebuffi2017icarl}$^\ast$ & 66.52 & 57.26 & 54.27 & 50.62 & 47.33 & 44.99 & 43.14 & 41.16 & 39.49 & -5.79 \\
Rebalance~\cite{hou2019learning}$^\ast$ & 66.66 & 61.42 & 57.29 & 53.02 & 48.85 & 45.68 & 43.06 & 40.56 & 38.35 & -6.93 \\
FSLL~\cite{mazumder2021few}$^\ast$ & 65.18 & 56.24 & 54.55 & 51.61 & 49.11 & 47.27 & 45.35 & 43.95 & 42.22 & -3.08 \\
iCaRL \cite{rebuffi2017icarl} & 64.10 & 53.28 & 41.69 & 34.13 & 27.93 & 25.06 & 20.41 & 15.48 & 13.73 & -31.55 \\
Rebalance \cite{hou2019learning} & 64.10 & 53.05 & 43.96 & 36.97 & 31.61 & 26.73 & 21.23 & 16.78 & 13.54 & -31.74 \\
TOPIC~\cite{cheraghian2021semantic} & 64.10 & 55.88 & 47.07 & 45.16 & 40.11 & 36.38 & 33.96 & 31.55 & 29.37 & -15.91 \\
F2M~\cite{shi2021overcoming} & 64.71 & 62.05 & 59.01 & 55.58 & 52.55 & 49.96 & 48.08 & 46.28 & 44.67 & -0.61 \\
\midrule 
% ---- euc distance measurements without training  --------
FSLL \cite{mazumder2021few} & 64.10 & 55.85 & 51.71 & 48.59 & 45.34 & 43.25 & 41.52 & 39.81 & 38.16 & -7.12 \\
%FSLL+SS \cite{mazumder2021few} & 66.76 & 55.52 & 52.20 & 49.17 & 46.23 & 44.64 & 43.07 & 41.20 & 39.57 & -5.71 \\
HardNet, $c=10\%$   
& 28.97	& 27.71 & 26.08 & 24.68	& 23.34 & 22.02 & 21.12 & 20.48 & 19.50 & -25.78 \\
HardNet, $c=20\%$   
& 37.42	& 35.29 & 33.22 & 31.32 & 29.51 & 27.80 & 26.54 & 25.28 & 24.16 & -21.12 \\
HardNet, $c=30\%$   
& 55.47	& 52.37 & 49.38 & 46.53 & 43.88 & 41.50 & 39.58 & 37.82 & 36.06	& -9.22 \\
HardNet, $c=40\%$   
& 57.52	& 53.85 & 50.62 & 47.74 & 44.90 & 42.64 & 40.76 & 38.95 & 37.07	& -8.21 \\
HardNet, $c=50\%$   
& \underbar{64.80}	& \underbar{60.77} & \underbar{56.95} & \underbar{53.53} & \underbar{50.40} & \underbar{47.82} & \underbar{45.93} & \underbar{43.95} & \underbar{41.91}	& -\underbar{3.37} \\
HardNet, $c=60\%$   
& 66.72	& 62.21 & 58.14 & 54.60 & 51.47 & 48.86 & 46.67 & 44.67 & 42.66	& -2.62 \\
HardNet, $c=70\%$   
& 68.27 & 63.52 & 59.45 & 55.89 & 52.91 & 50.30 & 48.27 & 46.25 & 44.22	& -1.06 \\
HardNet, $c=80\%$   
& 69.65	& 64.60 & 60.59 & 56.93 & 53.60 & 50.80 & 48.69 & 46.69 & 44.63	& -0.65 \\
HardNet, $c=90\%$ 
& 70.85 & 65.84 & 61.59 & 57.92 & 54.65 & 51.90 & 49.79 & 47.66 & 45.47 & +0.19 \\
HardNet, $c=93\%$   
& 71.22	& 66.20 & 62.00 & 58.34 & 55.04 & 52.34 & 50.22 & 48.07 & 46.04 & +0.76 \\
HardNet, $c=95\%$   
& 71.73	& 66.31 & 62.17 & 58.44 & 54.98	& 52.20 & 50.17 & 47.97 & 45.87	& +0.59 \\ 
HardNet, $c=97\%$   
& 71.85	& 66.48 & 62.29	& 58.62 & 55.36 & 52.55 & 50.60 & 48.43 & 46.22	& +0.94 \\
HardNet, $c=99\%$  
&71.95 & 66.83 & 62.75 & 59.09 & 55.92 & 53.03 & 50.78 & 48.52 & 46.31 & +1.03 \\
\midrule
% ---- layer4  --------
SoftNet, ~~$c=10\%$   
& 60.77	& 57.02 & 53.62 & 50.51 & 47.67 & 45.14 & 43.32 & 41.6 & 39.58 & -5.70 \\
SoftNet, ~~$c=20\%$   
& 64.67	& 60.69 & 57.15 & 53.77 & 50.76 & 48.28 & 46.24 & 44.23 & 42.31	& -2.97 \\
SoftNet, ~~$c=30\%$   
& 67.00 & 62.18 & 58.22 & 54.69 & 51.82 & 49.12 & 47.13 & 44.98 & 42.44 & -2.84 \\
SoftNet, ~~$c=40\%$   
& 67.50 & 63.11 & 59.29 & 55.61 & 52.53 & 49.85 & 47.85 & 45.84 & 43.85 & -1.43 \\
SoftNet, ~~$c=50\%$   
& 69.20 & 64.18 & 60.01 & 56.43 & 53.11 & 50.62 & 48.60 & 46.51 & 44.61 & -0.67 \\
SoftNet, ~~$c=60\%$ 
& 69.15	& 63.68 & 59.54 & 56.05 & 52.72 & 50.10 & 48.20 & 46.18 & 44.15 & -1.13 \\
SoftNet, ~~$c=70\%$ 
& 70.92 & 65.16 & 61.00 & 57.25 & 54.09 & 51.37 & 49.29 & 47.03 & 44.90 & -0.38 \\
SoftNet, ~~$c=80\%$ 
& 70.38 & 65.04 & 60.94 & 57.26 & 54.13 & 51.58 & 49.52 & 47.36 & 45.16 & -0.12 \\
SoftNet, ~~$c=90\%$ 
& 72.25	& 66.82 & 62.63 & 58.98 & 55.64 & 52.77 & 50.71 & 48.42 & 46.15 & +0.87 \\
SoftNet, ~~$c=93\%$ 
& 71.38	& 65.93 & 61.89 & 58.20 & 54.87 & 51.83 & 49.82 & 47.57 & 45.47 & +0.19 \\
SoftNet, ~~$c=95\%$ 
& 72.23 & 66.94 & 62.56 & 58.84 & 55.65 & 52.74 & 50.61 & 48.47 & 46.27 & +0.99 \\
SoftNet, ~~$c=97\%$ 
& 70.88	& 65.72 & 61.38 & 57.88 & 54.63 & 51.82 & 49.57 & 47.30 & 45.19	& -0.09 \\
SoftNet, ~~$c=99\%$ 
& \textbf{72.62} & \textbf{67.31} & \textbf{63.05} & \textbf{59.39}	& \textbf{56.00} & \textbf{53.23} & \textbf{51.06} & \textbf{48.83} & \textbf{46.63} & +\textbf{1.35}\\
\bottomrule
\end{tabular}
}
\label{tab:main_cifar100_5way_5shot_resnet18}
\end{center}
\end{table*}

==> soft-materials/6_exper/5_main_cifar100_temp.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy on CIFAR-100 for 5-way 5-shot FSCIL with varying temperatures $\tau$, fixed sparsity $c=0.9$ and $s=0.9$.}

\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{9}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\makecell{\textbf{The gap} \\ \textbf{with cRT}}}} \\ 
\cline{2-10}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &  \\
\midrule
cRT & 65.18 & 63.89 & 60.20 & 57.23 & 53.71 & 50.39 & 48.77 & 47.29 & 45.28 & - \\
\midrule
% ---- varying tau from 0.07 to 1.0 --------
SoftNet-c0.9-s0.9-$c_l0.102$, $\tau=0.07$  & 72.63 & 68.41 & 64.81 & 61.22 & 58.07 & 55.46 & 53.49 & 51.36 & 49.17 & +3.89 \\

SoftNet-c0.9-s0.9-$c_l0.102$, $\tau=0.1$   & 72.77 & 68.53 & 64.90 & 61.30 & 58.14 & 55.50 & 53.54 & 51.41 & 49.24 & +3.96 \\

SoftNet-c0.9-s0.9-$c_l0.102$, $\tau=\textbf{0.3}$   & \textbf{72.78} & \textbf{68.55} & \textbf{64.92} & \textbf{61.33} & \textbf{58.20} & \textbf{55.56} & \textbf{53.59} & \textbf{51.46} & \textbf{49.26} & +\textbf{3.98} \\

SoftNet-c0.9-s0.9-$c_l0.102$, $\tau=1.0$   & 72.52 & 68.33 & 64.77 & 61.17 & 58.05 & 55.39 & 53.48 & 51.39 & 49.14 & +3.85 \\
\midrule
% ---- varying tau from 0.07 to 1.0 --------
SoftNet-c0.9-s0.9-$c_l0.102$, $\tau=\textbf{0.3}$   & \textbf{72.78} & \textbf{68.55} & \textbf{64.92} & \textbf{61.33} & \textbf{58.20} & \textbf{55.56} & \textbf{53.59} & \textbf{51.46} & \textbf{49.26} & +\textbf{3.98} \\

SoftNet-c0.9-s0.9-$c_l0.5$, $~~~~\tau=0.3$   & 72.77 & 68.54 & 64.89 & 61.27 & 58.09 & 55.44 & 53.49 & 51.38 & 49.15 & +3.87 \\

SoftNet-c0.9-s0.9-$c_l0.7$, $~~~~\tau=0.3$   & 72.78 & 68.53 & 64.88 & 61.21 & 58.07 & 55.32 & 53.35 & 51.23 & 49.01 & +3.75 \\

SoftNet-c0.9-s0.9-$c_l0.9$, $~~~~\tau=0.3$   & 72.78 & 68.51 & 64.83 & 61.15 & 57.92 & 55.21 & 53.17 & 51.03 & 48.79 & +3.51 \\

\bottomrule
\end{tabular}}
\label{tab:cifar100_5way_5shot_temp}
\end{center}
\end{table*}

==> soft-materials/6_exper/5_main_cub_10way_5shot_hardnet_baseline.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy of ResNet18 on CUB-200-2011 for 10-way 5-shot incremental learning. \underbar{Underbar} denotes the comparable results with Baseline reported by \cite{shi2021overcoming}.}

\resizebox{0.96\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{11}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\makecell{\textbf{The gap} \\ \textbf{with cRT}}}} \\ 
\cline{2-12}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11   \\
\midrule
cRT [25] \cite{shi2021overcoming} & 80.83 & 78.51 & 76.12 & 73.93 & 71.46 & 68.96 & 67.73 & 66.75 & 64.22 & 62.53 & 61.08 & - \\
Joint-training \cite{shi2021overcoming} & 80.83 & 77.57 & 74.11 & 70.75 & 68.52 & 65.97 & 64.58 & 62.22 & 60.18 & 58.49 & 56.78 & -4.30 \\
Baseline \cite{shi2021overcoming} & 80.87 & 77.15 & 74.46 & 72.26 & 69.47 & 67.18 & 65.62 & 63.68 & 61.30 & 59.72 & 58.12 & -2.96 \\
\midrule
%iCaRL [40]∗ & 79.58 & 67.63 & 64.17 & 61.80 & 58.10 & 55.51 & 53.34 & 50.89 & 48.62 & 47.34 & 45.60 & -15.48 \\
%Rebalance [20]∗ & 80.94 & 70.32 & 62.96 & 57.19 & 51.06 & 46.70 & 44.03 & 40.15 & 36.75 & 34.88 & 32.09 & -28.99 \\
%FSLL [34]∗ & 80.83 & 77.38 & 72.37 & 71.84 & 67.51 & 65.30 & 63.75 & 61.16 & 59.05 & 58.03 & 55.82 & -5.26 \\
%iCaRL [40] & 68.68 & 52.65 & 48.61 & 44.16 & 36.62 & 29.52 & 27.83 & 26.26 & 24.01 & 23.89 & 21.16 & -39.92 \\
%Rebalance [20] & 68.68 & 57.12 & 44.21 & 28.78 & 26.71 & 25.66 & 24.62 & 21.52 & 20.12 &  20.06 & 19.87 & -41.21 \\
%TOPIC [47] & 68.68 & 62.49 & 54.81 & 49.99 & 45.25 & 41.40 & 38.35 & 35.36 & 32.22 & 28.31 & 26.28 & -34.80 \\
%FSLL [34] & 72.77 & 69.33 & 65.51 & 62.66 & 61.10 & 58.65 & 57.78 & 57.26 & 55.59 & 55.39 & 54.21 & -6.87 \\
%FSLL+SS [34] & 75.63 & 71.81 & 68.16 & 64.32 & 62.61 & 60.10 & 58.82 & 58.70 & 56.45 & 56.41 & 55.82 & -5.26 \\
%IDLVQ-C [8] & 77.37 & 74.72 & 70.28 & 67.13 & 65.34 & 63.52 & 62.10 & 61.54 & 59.04 & 58.68 & 57.81 & -3.27 \\
%F2M \cite{shi2021overcoming} & 81.07 & 78.16 & 75.57 & 72.89 & 70.86 & 68.17 & 67.01 & 65.26 & 63.36 & 61.76 & 60.26 & -0.82 \\
%\midrule
FSLL \cite{mazumder2021few} & 72.77 & 69.33 & 65.51 & 62.66 & 61.10 & 58.65 & 57.78 & 57.26 & 55.59 & 55.39 & 54.21 & -6.87 \\
%FSLL+SS \cite{mazumder2021few} & 75.63 & 71.81 & 68.16 & 64.32 & 62.61 & 60.10 & 58.82 & 58.70 & 56.45 & 56.41 & 55.82 & -5.26 \\
HardNet, $c=0.70$ & 74.09 &	71.13 &	67.22 &	63.75 &	61.85 &	59.29 &	58.36 &	57.47 &	55.47 &	54.92 &	54.17 &	-6.91 \\
HardNet, $c=0.80$ & 74.84 &	71.55 &	67.67 &	64.10 &	62.51 &	60.14 &	59.13 &	58.39 & 56.58 &	56.19 &	55.63 &	-5.45\\
HardNet, $c=0.90$ & 74.81 & 71.22 &	67.31 & 63.66 &	61.95 &	59.65 &	58.96 &	58.20 &	56.45 &	56.31 &	55.66 &	-5.42 \\
HardNet, $c=0.93$ & 75.16 & 71.29 &	67.36 &	63.85 &	62.05 &	59.64 &	58.89 &	58.04 &	56.33 &	56.05 &	55.59 &	-5.49 \\
HardNet, $c=0.95$ & 74.94 & 71.16 &	67.32 &	63.66 &	61.76 &	59.43 &	58.59 &	57.71 &	55.87 & 55.61 &	55.00 & -6.08 \\
HardNet, $c=0.97$ & 74.94 & 71.14 &	67.27 &	63.69 &	61.75 &	59.15 &	58.26 &	57.23 &	55.32 &	54.89 & 54.24 &	-6.84 \\
HardNet, $c=0.99$ & 74.78 & 71.17 &	57.08 & 63.40 &	61.39 & 58.84 & 57.82 & 56.67 &	54.80 &	54.26 & 53.49 &	-7.59 \\
\midrule
SoftNet,~~$c=0.70$ & 74.06 & 71.17 & 67.24 & 63.75 & 61.85 & 59.29 & 58.37 & 57.42 & 55.47 & 54.95 & 54.17 & -6.91 \\
SoftNet,~~$c=0.80$ & 74.79 & 71.53 & 67.65 & 64.13 & 62.49 & 60.09 & 59.08 & 58.36 & 56.54 & 56.22 & 55.58 & -5.50 \\
SoftNet,~~$c=0.90$ & 74.76 & 71.23 & 67.29 & 63.65 & 61.93 & 59.65 & 58.99 & 58.20 & 56.49 & 56.29 & 55.63 & -5.45 \\
SoftNet,~~$c=0.93$ & 75.14 & 71.26 & 67.31 & 63.80 & 62.09 & 59.66 & 58.88 & 58.01 & 56.36 & 56.08 & 55.54 & -5.54 \\
SoftNet,~~$c=0.95$ & 74.90 & 71.17 & 67.35 & 63.64 & 61.75 & 59.39 & 58.57 & 57.69 & 55.91 & 55.59 & 54.98 & -6.10 \\
SoftNet,~~$c=0.97$ & 74.93 & 71.18 & 67.27 & 63.68 & 61.75 & 59.18 & 58.21 & 57.19 & 55.31 & 54.89 & 54.23 & -6.85 \\
SoftNet,~~$c=0.99$ & 74.79 & 71.12 & 57.11 & 63.37 & 61.37 & 58.79 & 57.79 & 56.71 & 54.81 & 54.26 & 53.52 & -7.56 \\
\bottomrule
\end{tabular}}
\label{tab:cub_10way_5shot}
\end{center}
\end{table*}

==> soft-materials/6_exper/5_main_miniImageNet_5way_5shot_hardnet_baseline.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy of ResNet18 on miniImageNet for 5-way 5-shot incremental learning. \underbar{Underbar} denotes the comparable results with baseline. $\ast$ denotes results reported from \cite{shi2021overcoming}.}

\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{9}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\makecell{\textbf{The gap} \\ \textbf{with cRT}}}} \\ 
\cline{2-10}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &  \\
\midrule
cRT \cite{shi2021overcoming} & 67.30 & 64.15 & 60.59 & 57.32 & 54.22 & 51.43 & 48.92 & 46.78 & 44.85 & - \\
Joint-training \cite{shi2021overcoming} & 67.30 & 62.34 & 57.79 & 54.08 & 50.93 & 47.65 & 44.64 & 42.61 & 40.29 & -4.56 \\
Baseline \cite{shi2021overcoming} & 67.30 & 63.18 & 59.62 & 56.33 & 53.28 & 50.50 & 47.96 & 45.85 & 43.88 & -0.97 \\
\midrule
iCaRL \cite{rebuffi2017icarl}$^\ast$ & 67.35 & 59.91 & 55.64 & 52.60 & 49.43 & 46.73 & 44.13 & 42.17 & 40.29 & -4.56 \\
Rebalance \cite{hou2019learning}$^\ast$ & 67.91 & 63.11 & 58.75 & 54.83 & 50.68 & 47.11 & 43.88 & 41.19 & 38.72 & -6.13 \\
FSLL \cite{mazumder2021few}$^\ast$ & 67.30 & 59.81 & 57.26 & 54.57 & 52.05 & 49.42 & 46.95 & 44.94 & 42.87 & -1.11 \\
iCaRL \cite{rebuffi2017icarl} & 61.31 & 46.32 & 42.94 & 37.63 & 30.49 & 24.00 & 20.89 & 18.80 & 17.21 & -27.64 \\
Rebalance \cite{hou2019learning} & 61.31 & 47.80 & 39.31 & 31.91 & 25.68 & 21.35 & 18.67 & 17.24 & 14.17 & -30.68 \\
TOPIC \cite{cheraghian2021semantic} & 61.31 & 50.09 & 45.17 & 41.16 & 37.48 & 35.52 & 32.19 & 29.46 & 24.42 & -20.43 \\
IDLVQ-C \cite{chen2020incremental} & 64.77 & 59.87 & 55.93 & 52.62 & 49.88 & 47.55 & 44.83 & 43.14 & 41.84 & -3.01 \\
F2M \cite{shi2021overcoming} & 67.28 & 63.80 & 60.38 & 57.06 & 54.08 & 51.39 & 48.82 & 46.58 & 44.65 & -0.20 \\
\midrule 
FSLL \cite{mazumder2021few} & 66.48 & 61.75 & 58.16 & 54.16 & 51.10 & 48.53 & 46.54 & 44.20 & 42.28 & -2.57 \\
HardNet, $c=10\%$  
& 9.70 & 8.46 & 8.13 & 7.67 & 7.35 & 6.78 & 6.55 & 6.3 & 5.8 & -39.05 \\
HardNet, $c=20\%$  
& 24.95 & 22.20 & 20.66 & 19.39 & 18.32 & 17.41 & 16.64 & 15.79 & 15.28 & -29.57 \\
HardNet, $c=30\%$  
& 44.08	 & 40.66 & 38.24 & 36.06 & 33.65 & 31.84 & 30.25 & 29.01 & 28.02 & -16.83 \\
HardNet, $c=40\%$  
& 37.05 & 34.94 & 32.25 & 30.72 & 29.09 & 27.53 & 25.84 & 24.76 & 23.71 & -21.14 \\
HardNet, $c=50\%$  
& \underbar{65.13} & \underbar{60.37} & \underbar{56.12} & \underbar{53.17} & \underbar{50.17} & \underbar{47.74} & \underbar{45.34} & \underbar{43.35} & \underbar{42.13}	& -\underbar{2.72} \\
HardNet, $c=60\%$  
& 73.32 & 67.77 & 63.46 & 60.13 & 57.13 & 50.36 & 47.88 & 46.05 & 44.59 & -0.26 \\
HardNet, $c=70\%$  
& 71.75	& 66.66 & 62.19 & 58.85 & 55.74 & 52.82 & 50.14 & 48.45 & 47.01 & +2.16 \\
HardNet, $c=80\%$  
& 69.73 & 64.46 & 60.42 & 57.09 & 54.09 & 51.18 & 48.76 & 46.81	& 45.66 & +0.81 \\
HardNet, $c=90\%$  
& 64.68	& 59.80 & 55.70 & 52.82 & 50.01 & 47.30 & 45.17 & 43.34 & 42.09	& -2.76 \\
HardNet, $c=93\%$  
& 67.17	& 61.74 & 57.53 & 54.43 & 51.52 & 48.86 & 46.42 & 44.68 & 43.43	& -1.42 \\
HardNet, $c=95\%$  
& 64.72	& 60.13 & 56.05 & 53.25 & 50.20 & 47.62 & 45.11 & 43.40 & 42.33	& -2.52 \\
HardNet, $c=97\%$  
& 63.92	& 58.85 & 55.12	& 52.16 & 49.44 & 46.78 & 44.48 & 42.68 & 41.52	& -3.33 \\
HardNet, $c=99\%$  
& 67.28 & 62.17 & 58.06 & 55.05 & 52.01 & 49.12 & 46.92 & 45.07 & 43.90 & -0.95 \\
\midrule 
% ------------ layer 4------------------------
SoftNet, ~~$c=10\%$  
& 62.75 & 58.26 & 53.80 & 50.82 & 47.68 & 44.86 & 42.05 & 39.86 & 38.15 & -6.70 \\
SoftNet, ~~$c=20\%$  
& 68.33	& 62.76 & 58.60 & 55.25 & 52.07 & 49.36 & 46.48 & 44.21 & 42.52 & -2.33 \\
SoftNet, ~~$c=30\%$  
& 72.20 & 66.92 & 62.56 & 59.16 & 56.07 & 53.10	& 50.59 & 48.46 & 47.03 & +2.18 \\
SoftNet, ~~$c=40\%$  
& 72.58	& 67.34 & 62.91 & 59.65 & 56.72	& 54.00 & 51.46 & 49.39 & 48.11 & +3.26 \\
SoftNet, ~~$c=50\%$  
& 72.83	& 67.23 & 62.82 & 59.41 & 56.44 & 53.55 & 50.92 & 48.99 & 47.60 & +2.75 \\
SoftNet, ~~$c=60\%$  
& 73.83	& 67.78 & 63.46 & 60.21 & 57.27 & 54.42 & 51.74 & 49.94 & 48.57 & +3.72 \\
SoftNet, ~~$c=70\%$  
& 75.15 & 69.06	& 64.79	& 61.40	& 58.38	& 55.49 & 52.87 & 50.89 & 49.69 & +4.84 \\
SoftNet, ~~$c=80\%$  
& 76.63	& 70.13	& 65.92 & 62.52 & \textbf{59.49} & \textbf{56.56} & 53.71 & 51.72 & \textbf{50.48} & +\textbf{5.63} \\
SoftNet, ~~$c=90\%$  
& 77.00 & \textbf{70.38} & 65.94 & 62.45 & 59.32 & 56.25 & \textbf{53.76} & \textbf{51.75} & 50.39 & +5.54 \\
SoftNet, ~~$c=93\%$  
& 73.97 & 67.39 & 63.35 & 59.90 & 56.89 & 54.18 & 51.61 & 49.71 & 48.45 & +3.60 \\
SoftNet, ~~$c=95$\%  
& 76.22	& 69.64 & 65.22 & 61.91 & 58.84 & 55.75 & 53.07	& 51.18 & 49.84 & +4.99 \\
SoftNet, ~~$c=97\%$  
& \textbf{77.17} & 70.32 & \textbf{66.15} & \textbf{62.55} & 59.48 & 56.46 & 53.71 & 51.68 & 50.24 & +5.39 \\
SoftNet, ~~$c=99\%$  
& 76.80 & 69.79 & 65.44 & 62.01 & 58.87 & 55.94 & 53.21 & 51.25 & 50.04 & +5.19 \\
\bottomrule
\end{tabular}}
\label{tab:miniImageNet_5way_5shot_baseline}
\end{center}
\end{table*}

==> soft-materials/6_exper/5_main_miniImageNet_5way_5shot_layer.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy of ResNet18 on miniImageNet for 5-way 5-shot incremental learning. The layer-wise inspection with fixed $c=97 \%$. \textit{all} denotes that all minor weights $\bm{m}_{\text{minor}}$ of the entire layers were trained while only \textit{conv}$\ast$x trained.}

\resizebox{0.86\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{9}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\thead{\textbf{The gap} \\ \textbf{with cRT}}}} \\ 
%\vspace{0.005in}
\cline{2-10}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &  \\
\midrule
cRT \cite{shi2021overcoming} & 67.30 & 64.15 & 60.59 & 57.32 & 54.22 & 51.43 & 48.92 & 46.78 & 44.85 & - \\
%Joint-training \cite{shi2021overcoming} & 67.30 & 62.34 & 57.79 & 54.08 & 50.93 & 47.65 & 44.64 & 42.61 & 40.29 & -4.56 \\
%Baseline \cite{shi2021overcoming} & 67.30 & 63.18 & 59.62 & 56.33 & 53.28 & 50.50 & 47.96 & 45.85 & 43.88 & -0.97 \\
\midrule

% ------------ layer 4------------------------
%SoftNet, ~~$c=0.10$  
%& 62.75 & 58.26 & 53.80 & 50.82 & 47.68 & 44.86 & 42.05 & 39.86 & 38.15 & -6.7 \\
%SoftNet, ~~$c=0.20$  
%& 68.33	& 62.76 & 58.60 & 55.25 & 52.07 & 49.36 & 46.48 & 44.21 & 42.52 & -2.33 \\
%SoftNet, ~~$c=0.30$  
%& 72.20 & 66.92 & 62.56 & 59.16 & 56.07 & 53.10	& 50.59 & 48.46 & 47.03 & +2.18 \\
%SoftNet, ~~$c=0.40$  
%& 72.58	& 67.34 & 62.91 & 59.65 & 56.72	& 54.00 & 51.46 & 49.39 & 48.11 & +3.26 \\
%SoftNet, ~~$c=0.50$  
%& 72.83	& 67.23 & 62.82 & 59.41 & 56.44 & 53.55 & 50.92 & 48.99 & 47.60 & +2.75 \\
%SoftNet, ~~$c=0.60$  
%& 73.83	& 67.78 & 63.46 & 60.21 & 57.27 & 54.42 & 51.74 & 49.94 & 48.57 & +3.72 \\
%SoftNet, ~~$c=0.70$  
%& 75.15 & 69.06	& 64.79	& 61.40	& 58.38	& 55.49 & 52.87 & 50.89 & 49.69 & +4.84 \\
%SoftNet, ~~$c=0.80$  
%& 76.63	& 70.13	& 65.92 & 62.52 & \textbf{59.49} & \textbf{56.56} & 53.71 & 51.72 & \textbf{50.48} & +\textbf{5.63} \\
%SoftNet, ~~$c=0.90$  
%& 77.00 & \textbf{70.38} & 65.94 & 62.45 & 59.32 & 56.25 & \textbf{53.76} & \textbf{51.75} & 50.39 & +5.54 \\
%SoftNet, ~~$c=0.93$  
%& 73.97 & 67.39 & 63.35 & 59.90 & 56.89 & 54.18 & 51.61 & 49.71 & 48.45 & +3.60 \\
%SoftNet, ~~$c=0.95$  
%& 76.22	& 69.64 & 65.22 & 61.91 & 58.84 & 55.75 & 53.07	& 51.18 & 49.84 & +4.99 \\
%SoftNet, ~conv1  
%& \textbf{77.17} & -  & - & - & - & - & - & - & - & -  \\
SoftNet, ~Conv2x  
& 77.17 & 70.29 & 66.09 & 62.54 & 59.44 & 56.43 & 53.68 & 51.60 & 50.19 & +5.34 \\
SoftNet, ~Conv3x  
& 77.17 & 70.30	& 66.05 & 62.51 & 59.42 & 56.44 & 53.70 & 51.59 & 50.15 & +5.30 \\
SoftNet, ~Conv4x  
& 77.17 & 70.30 & 66.08 & 62.54 & 59.45 & 56.46 & 53.70 & 51.59 & 50.17& +5.32 \\
SoftNet, ~Conv5x  
& \textbf{77.17} & \textbf{70.32} & \textbf{66.15} & \textbf{62.55} & \textbf{59.48} & \textbf{56.46} & \textbf{53.71} & \textbf{51.68} & \textbf{50.24} & +\textbf{5.39} \\
SoftNet, ~All  
& 77.17 & 65.09 & 55.25 & 45.92 & 38.20 & 33.37 & 29.52 & 27.66 & 25.64 & -19.21  \\
%SoftNet, ~~$c=0.99$  
%& 76.80 & 69.79 & 65.44 & 62.01 & 58.87 & 55.94 & 53.21 & 51.25 & 50.04 & +5.19 \\
\bottomrule
\end{tabular}
}
\label{tab:miniImageNet_5way_5shot_layerwise}
\end{center}
% \vspace{-0.1in}
\end{table*}

==> soft-materials/6_exper/5_main_plots_cifar_hardnet_cap.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    %\setlength{\tabcolsep}{-0pt}{%
    \begin{tabular}{ccc}
    \includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/layer3_hardnet_cap_acc_cifar100.pdf} & &
    %\includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/avg_acc_0.1.pdf} & &
    \includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/layer3_hardnet_new_cap_acc_cifar100.pdf} \\
    
    \makecell{\small{(a) from $c=0.80$ to $c= 0.99$ with fixed $c_l=0.102$}} & &
    \makecell{\small{(b) from $c_l=1.01$ to $c_l=1.50$ with fixed $c=0.95$}} \\
    %\makecell{\small{(c) $\tau = 0.3$}}\\
    \end{tabular}
    %\end{adjustbox}
    \caption{\small \textbf{SoftNet on CIFAR-100 for 5-way 5-shot FSCIL:} (a) the effect of $c$ with fixed $c_l=0.102$ and (b) the effect of $c_l$ with fixed $c=0.95$. $\bigtriangledown$ and $\square$ denote base class and novel class performances, respectively.}
    \label{fig:hardnet_cap_cifar100}
\end{figure*}

==> soft-materials/6_exper/5_main_plots_cifar_temp.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    %\setlength{\tabcolsep}{-0pt}{%
    \begin{tabular}{ccc}
    \includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/overall_avg_acc_cifar100.pdf} & &
    %\includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/avg_acc_0.1.pdf} & &
    \includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/layer3_cap_acc_cifar100.pdf} \\
    
    \makecell{\small{(a) from $\tau = 0.07$ to $\tau = 1.0$ with fixed $c_l=0.102$}} & &
    \makecell{\small{(b) from $c_l=0.102$ to $c_l=0.9$ with $\tau = 0.3$}} \\
    %\makecell{\small{(c) $\tau = 0.3$}}\\
    \end{tabular}
    %\end{adjustbox}
    \caption{\small \textbf{SoftNet on CIFAR-100 for 5-way 5-shot FSCIL:} (a) the effect of $\tau$ with fixed $c_l=0.102$ and (b) the effect of $c_l$ with fixed $\tau=0.3$. $\bigtriangledown$ and $\square$ denote base class and novel class performances, respectively.}
    \label{fig:softnet_temp_cifar100}
\end{figure*}

==> soft-materials/6_exper/5_main_plots_loss_lens.tex <==
\begin{figure*}[ht]
    \centering
    \setlength{\tabcolsep}{-6pt}{%
    \begin{tabular}{cc}
    
    %\includegraphics[width=0.37\textwidth]{images/loss_lens/loss_func_surface_3D_epoch30.pdf} & 
    
    \includegraphics[width=0.49\textwidth]{images/loss_lens/loss_func_surface_3D_epoch70.pdf} &

    \includegraphics[width=0.49\textwidth]{images/loss_lens/loss_func_surface_3D_epoch100.pdf} \\ 
    
    % plot captions
    \small (a) epoch=70, $c=10.0\%$ & \small (b) epoch=100, $c=10.0\%$  \\
    \end{tabular}
    }
    \caption{\small \textbf{Loss landscapes of } \textcolor{teal}{DenseNet}, \textcolor{red}{HardNet}, \textbf{and} \textcolor{cyan}{SoftNet}: Subnetworks provide a more flat global minimum than dense neural networks. To demonstrate the loss landscapes, we trained a simple three-layered, fully connected model (fc-4-25-30-3) on the Iris Flower dataset (which is three classification problem) for 100 epochs.}
    
    \label{fig:main_plot_loss_lens}
\end{figure*}

==> soft-materials/6_exper/5_main_plots_soft_hard.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    %\setlength{\tabcolsep}{-0pt}{%
    \begin{tabular}{cc}
    \includegraphics[height=4.6cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/layer3_softnet_new_cap_acc_cifar100.pdf} & 
    \includegraphics[height=4.6cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/miniImageNet/layer3_softnet_new_cap_acc_miniImageNet.pdf} \\
    
    
    \makecell{\small{(a) CIFAR-100}} &
    \makecell{\small{(b) miniImageNet}} \\
    %\makecell{\small{(c) $\tau = 0.3$}}\\
    \end{tabular}
    %\end{adjustbox}
    \caption{\small \textbf{Classification accuracy of HardNet v.s SoftNet on CIFAR-100 and miniImageNet for 5-way 5-shot FSCIL:} the overall performance depends on capacity $c$ and the softness of subnetwork and $\bigcirc$, $\bigtriangledown$, and $\square$ denote overall, base class, and novel class performances respectively. The new session performances $\square$ of SoftNet are better than those of HardNet while least forgetting base session knowledge $\bigcirc$.}
    \label{fig:hardnet_softnet}
\end{figure*}

==> soft-materials/6_exper/5_main_res18_20_cifar100_5way_5shot.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy of ResNet18, 20, 32, and 50 on CIFAR-100 for 5-way 5-shot FSCIL.}

\resizebox{0.82\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{9}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\thead{\textbf{The gap} \\ \textbf{with cRT}}}} \\ 
%\vspace{.005in}
\cline{2-10} 
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &  \\
\midrule
ResNet18, cRT \cite{shi2021overcoming} & 65.18 & 63.89 & 60.20 & 57.23 & 53.71 & 50.39 & 48.77 & 47.29 & 45.28 & - \\
%ResNet18, cRT  & 65.18 & 63.89 & 60.20 & 57.23 & 53.71 & 50.39 & 48.77 & 47.29 & 45.28 & - \\
%ResNet18, Joint-training \cite{shi2021overcoming} & 65.18 & 61.45 & 57.36 & 53.68 & 50.84 & 47.33 & 44.79 & 42.62 & 40.08 & -5.20 \\
%ResNet18, Baseline \cite{shi2021overcoming} & 65.18 & 61.67 & 58.61 & 55.11 & 51.86 & 49.43 & 47.60 & 45.64 & 43.83 & -1.45 \\
\midrule
%iCaRL~\cite{rebuffi2017icarl}$^\ast$ & 66.52 & 57.26 & 54.27 & 50.62 & 47.33 & 44.99 & 43.14 & 41.16 & 39.49 & -5.79 \\
%Rebalance~\cite{hou2019learning}$^\ast$ & 66.66 & 61.42 & 57.29 & 53.02 & 48.85 & 45.68 & 43.06 & 40.56 & 38.35 & -6.93 \\
%FSLL~\cite{mazumder2021few}$^\ast$ & 65.18 & 56.24 & 54.55 & 51.61 & 49.11 & 47.27 & 45.35 & 43.95 & 42.22 & -3.08 \\
%iCaRL \cite{rebuffi2017icarl} & 64.10 & 53.28 & 41.69 & 34.13 & 27.93 & 25.06 & 20.41 & 15.48 & 13.73 & -31.55 \\
%Rebalance \cite{hou2019learning} & 64.10 & 53.05 & 43.96 & 36.97 & 31.61 & 26.73 & 21.23 & 16.78 & 13.54 & -31.74 \\
%TOPIC~\cite{cheraghian2021semantic} & 64.10 & 55.88 & 47.07 & 45.16 & 40.11 & 36.38 & 33.96 & 31.55 & 29.37 & -15.91 \\
%F2M~\cite{shi2021overcoming} & 64.71 & 62.05 & 59.01 & 55.58 & 52.55 & 49.96 & 48.08 & 46.28 & 44.67 & -0.61 \\
%\midrule
%FSLL \cite{mazumder2021few} & 64.10 & 55.85 & 51.71 & 48.59 & 45.34 & 43.25 & 41.52 & 39.81 & 38.16 & -7.12 \\
%ResNet18, HardNet, $c=0.10$   
%& 28.97	& 27.71 & 26.08 & 24.68	& 23.34 & 22.02 & 21.12 & 20.48 & 19.50 & -25.78 \\
%ResNet18, HardNet, $c=0.20$   
%& 37.42	& 35.29 & 33.22 & 31.32 & 29.51 & 27.80 & 26.54 & 25.28 & 24.16 & -21.12 \\
%ResNet18, HardNet, $c=0.30$   
%& 55.47	& 52.37 & 49.38 & 46.53 & 43.88 & 41.50 & 39.58 & 37.82 & 36.06	& -9.22 \\
%ResNet18, HardNet, $c=0.40$   
%& 57.52	& 53.85 & 50.62 & 47.74 & 44.90 & 42.64 & 40.76 & 38.95 & 37.07	& -8.21 \\
%ResNet18, HardNet, $c=0.50$   
%& \underbar{64.80}	& \underbar{60.77} & \underbar{56.95} & \underbar{53.53} & \underbar{50.40} & \underbar{47.82} & \underbar{45.93} & \underbar{43.95} & \underbar{41.91}	& -\underbar{3.37} \\
%ResNet18, HardNet, $c=0.60$   
%& 66.72	& 62.21 & 58.14 & 54.60 & 51.47 & 48.86 & 46.67 & 44.67 & 42.66	& -2.62 \\
%ResNet18, HardNet, $c=0.70$   
%& 68.27 & 63.52 & 59.45 & 55.89 & 52.91 & 50.30 & 48.27 & 46.25 & 44.22	& -1.06 \\
%ResNet18, HardNet, $c=0.80$   
%& 69.65	& 64.60 & 60.59 & 56.93 & 53.60 & 50.80 & 48.69 & 46.69 & 44.63	& -0.65 \\
%ResNet18, HardNet, $c=0.90$ 
%& 70.85 & 65.84 & 61.59 & 57.92 & 54.65 & 51.90 & 49.79 & 47.66 & 45.47 & +0.19 \\
%ResNet18, HardNet, $c=0.93$   
%& 71.22	& 66.20 & 62.00 & 58.34 & 55.04 & 52.34 & 50.22 & 48.07 & 46.04 & +0.76 \\
%ResNet18, HardNet, $c=0.95$   
%& 71.73	& 66.31 & 62.17 & 58.44 & 54.98	& 52.20 & 50.17 & 47.97 & 45.87	& +0.59 \\ 
%ResNet18, HardNet, $c=0.97$   
%& 71.85	& 66.48 & 62.29	& 58.62 & 55.36 & 52.55 & 50.60 & 48.43 & 46.22	& +0.94 \\
%ResNet18, HardNet, $c=0.99$  
%&71.95 & 66.83 & 62.75 & 59.09 & 55.92 & 53.03 & 50.78 & 48.52 & 46.31 & +1.03 \\
%\midrule
% ---- layer4  --------
%ResNet18, SoftNet, ~~$c=0.10$   
%& 60.77	& 57.02 & 53.62 & 50.51 & 47.67 & 45.14 & 43.32 & 41.6 & 39.58 & -5.7 \\
%ResNet18, SoftNet, ~~$c=0.20$   
%& 64.67	& 60.69 & 57.15 & 53.77 & 50.76 & 48.28 & 46.24 & 44.23 & 42.31	& -2.97 \\
%ResNet18, SoftNet, ~~$c=0.30$   
%& 67.00 & 62.18 & 58.22 & 54.69 & 51.82 & 49.12 & 47.13 & 44.98 & 42.44 & -2.84 \\
%ResNet18, SoftNet, ~~$c=0.40$   
%& 67.50 & 63.11 & 59.29 & 55.61 & 52.53 & 49.85 & 47.85 & 45.84 & 43.85 & -1.43 \\
%ResNet18, SoftNet, ~~$c=0.50$   
%& 69.20 & 64.18 & 60.01 & 56.43 & 53.11 & 50.62 & 48.60 & 46.51 & 44.61 & -0.67 \\
%ResNet18, SoftNet, ~~$c=0.60$ 
%& 69.15	& 63.68 & 59.54 & 56.05 & 52.72 & 50.10 & 48.20 & 46.18 & 44.15 & -1.13 \\
ResNet18, SoftNet, ~~$c=70\%$ 
& 70.92 & 65.16 & 61.00 & 57.25 & 54.09 & 51.37 & 49.29 & 47.03 & 44.90 & -0.38 \\
%ResNet18, SoftNet, ~~$c=0.80$ 
%& 70.38 & 65.04 & 60.94 & 57.26 & 54.13 & 51.58 & 49.52 & 47.36 & 45.16 & -0.12 \\
~~~~~~~~~~~~~~~~SoftNet, ~~$c=90\%$ 
& 72.25	& 66.82 & 62.63 & 58.98 & 55.64 & 52.77 & 50.71 & 48.42 & 46.15 & +0.87 \\
%ResNet18, SoftNet, ~~$c=0.93$ 
%& 71.38	& 65.93 & 61.89 & 58.20 & 54.87 & 51.83 & 49.82 & 47.57 & 45.47 & +0.19 \\
%ResNet18, SoftNet, ~~$c=0.95$ 
%& 72.23 & 66.94 & 62.56 & 58.84 & 55.65 & 52.74 & 50.61 & 48.47 & 46.27 & +0.99 \\
%ResNet18, SoftNet, ~~$c=0.97$ 
%& 70.88	& 65.72 & 61.38 & 57.88 & 54.63 & 51.82 & 49.57 & 47.30 & 45.19	& -0.09 \\
~~~~~~~~~~~~~~~~SoftNet, ~~$c=99\%$ 
& 72.62 & 67.31 & 63.05 & 59.39	& 56.00 & 53.23 & 51.06 & 48.83 & 46.63 & +1.35\\
\midrule


% ---- euc distance measurements without training  --------
%ResNet20, HardNet, $c=0.10$   
%& 53.50  & 50.52 & 47.79 & 45.11 & 42.57 & 40.38 & 38.88 & 37.43 & 35.69 & -9.59 \\
%ResNet20, HardNet, $c=0.20$   
%& 61.83 & 58.24 & 55.17 & 51.92 & 49.07 & 46.68 & 45.02 & 43.31 & 41.40 & -3.88 \\

%ResNet20, HardNet, $c=0.30$   
%& \underbar{66.68} & \underbar{62.81} &  \underbar{59.54} & \underbar{56.12} & \underbar{53.21} & \underbar{50.52} & \underbar{48.85} & \underbar{46.93} & \underbar{44.84} & -\underbar{0.44} \\
%ResNet20, HardNet, $c=0.40$   
%& 68.31 & 64.17 & 60.72 & 57.19 & 54.26 & 51.79 & 50.13 & 48.01 & 45.93 & +0.65 \\
%ResNet20, HardNet, $c=0.50$   
%& 70.73 & 66.56 & 63.10 & 59.59 & 56.58 & 53.87 & 51.86 & 49.72 & 47.46 & +2.18 \\
%ResNet20, HardNet, $c=0.60$   
%& 71.90	& 67.64 & 63.84 & 60.22 & 57.06 & 54.30 & 52.53 & 50.53 & 48.34 & +3.06 \\
%ResNet20, HardNet, $c=0.70$   
%& 71.41	& 67.44 & 63.76 & 60.02 & 56.84 & 54.14 & 52.54 & 50.42 & 48.24 & +2.96 \\
%ResNet20, HardNet, $c=0.80$   
%& 71.97 & 67.65 & 63.93 & 60.14 & 57.12 & 54.44 & 52.72 &50.67	& 48.43 & +3.15 \\
%ResNet20, HardNet, $c=0.90$ 
%& 71.82 & 67.73 & 64.21 & 60.44 & 57.44 & 54.93 & 53.14 & 51.03	& 48.86 & +3.58 \\
%ResNet20, HardNet, $c=0.93$   
%& 72.28 & 67.99 & 64.48 & 60.83 & 57.64 & 55.16 & 53.27 & 51.11	& 48.93 & +3.65 \\
%ResNet20, HardNet, $c=0.95$   
%& 72.13 & 68.14 & 64.50 & 60.74 & 57.68 & 55.12 & 53.17 & 51.23	& 48.97 & +3.69 \\ 
%ResNet20, HardNet, $c=0.97$   
%& 71.90	& 67.81 & 64.11 & 60.24 & 57.14 & 54.41 & 52.74 & 50.71 & 48.67 & +3.39 \\
%\midrule
% ---- layer3  --------
%ResNet20, SoftNet, $c=0.10$   
%& 53.13 & 49.73 & 46.85 & 44.01 & 41.54 & 39.45 & 37.84 & 36.30 & 34.62 & -10.66 \\
%ResNet20, SoftNet, $c=0.20$   
%& 60.15 & 56.25	& 53.26 & 50.16 & 47.46 & 45.23 & 43.75 & 41.84 & 39.90 & -5.38 \\
%ResNet20, SoftNet, ~~$c=0.30$   
%& 64.65	& 59.99 & 56.65 & 53.45 & 50.42 & 48.02 & 46.48 & 44.61 & 42.43 & -2.85 \\
%ResNet20, SoftNet, $c=0.40$   
%& 66.77	& 62.55 & 59.35 & 55.63 & 52.70 & 50.21 & 48.54 & 46.60 & 44.50 & -0.78 \\
%ResNet20, SoftNet, $c=0.50$   
%& 68.20 & 64.21 & 60.78 & 57.15 & 54.20 & 51.53 & 49.84 & 47.92 & 45.84 & +0.56 \\
%ResNet20, SoftNet, $c=0.60$ 
%& 68.63	& 64.76 & 61.00 & 57.53 & 54.56 & 52.11 & 50.34 & 48.41 & 46.30 & +1.02 \\
ResNet20, SoftNet, ~~$c=70\%$ 
& 70.38	& 66.16 & 62.63 & 58.93 & 55.81 & 53.11 & 51.38 & 49.29 & 47.08 & +1.80 \\
%ResNet20, SoftNet, $c=0.80$ 
%& 70.87	& 66.47 & 62.85 & 59.28 & 56.27 & 53.84 & 52.01 & 50.16 & 48.01 & +2.73 \\
~~~~~~~~~~~~~~~~SoftNet, ~~$c=90\%$ 
& 72.63 & 68.60 & 64.96 & 61.25 & 57.98 & 55.32 & 53.48 & 51.46 & 49.20 & +3.92 \\
%ResNet20, SoftNet, $c=0.93$ 
%& 72.53 & 68.45 & 64.59 & 60.80 & 57.48 & 54.91 & 53.19 & 51.03 & 48.83 & +3.55 \\
%ResNet20, SoftNet, $c=0.95$ 
%& 72.58 & 68.30 & 64.57 & 60.83 & 57.67 & 54.86 & 53.11 & 51.21 & 49.06 & +3.78 \\
%ResNet20, SoftNet, $c=0.97$ 
%& \textbf{72.80} & 68.46 & 64.61 & 60.90 & 57.63 & 54.95 & 53.26 & 51.12 & 48.95 & +3.67 \\
~~~~~~~~~~~~~~~~SoftNet, ~~$c=99\%$ 
& 71.78	& 67.79 & 63.86 & 60.07 & 57.05 & 54.32 & 52.34 & 50.28 & 48.11 & +2.83 \\ \midrule 

%---------------------------
%ResNet32, SoftNet, ~~$c=0.80$ 
%& 73.92 & 69.58 & 65.74 & 61.83 & 58.43  & 55.68  & 53.53  & 51.41  & 48.98  & +3.70 \\ 

ResNet32, SoftNet, ~~$c=90\%$ 
& 75.47 & 70.84 & 66.84 & 63.01 & 59.69  & 56.86  & 54.75  & 52.70  & 50.36  & +5.08\\ 

~~~~~~~~~~~~~~~~SoftNet, ~~$c=93\%$ 
& 75.35 & 71.22 & 67.25 & 63.25 & 60.05  & 57.24  & 55.16  & 53.01  & 50.76  & +5.48\\ 

~~~~~~~~~~~~~~~~SoftNet, ~~$c=95\%$ 
& 74.67 & 70.32 & 66.31 & 62.61 & 59.29  & 56.54  & 54.52  & 52.30  & 50.05  & +4.77\\ 

%ResNet32, SoftNet, ~~$c=0.97$ 
%& 75.18 & 70.49 & 66.66 & 62.84 & 59.47  & 56.56  & 54.59  & 52.45  & 50.24  & +4.96\\ 

%ResNet32, SoftNet, ~~$c=0.99$ 
%& 75.17 & 70.76 & 67.03 & 62.98 & 59.67  & 56.84  & 54.86  & 52.72  & 50.59  & +5.01\\ \midrule

\midrule 
%ResNet50, SoftNet, ~~$c=0.50$ 
%& 77.00	& 72.39  & 68.37 & 64.42 & 60.94  & 57.86  & 55.50  & 53.30  & 51.08 &  +5.80 \\

%ResNet50, SoftNet, ~~$c=0.60$ 
%& 77.90	& 73.48  & 69.41 & 65.40 & 61.97  & 58.76  & 56.45  & 54.04  & 51.88 &  +6.60\\

ResNet50, SoftNet, ~~$c=70\%$ 
& 76.20	& 71.82  & 67.90 & 64.17 & 60.91  & 57.89  & 55.72  & 53.20  & 50.87 &  +5.59 \\

~~~~~~~~~~~~~~~~SoftNet, ~~$c=80\%$ 
& \textbf{78.20}	& \textbf{73.32}  &  \textbf{69.22} & \textbf{65.43} & \textbf{62.09}  & \textbf{59.08}  & \textbf{56.80}  & \textbf{54.45}  & \textbf{52.18} &  +\textbf{6.90}\\

~~~~~~~~~~~~~~~~SoftNet, ~~$c=90\%$ 
& 77.67	& 72.73  &  68.50 & 64.57 & 61.08  & 58.06  & 55.70  & 53.37  & 51.20  &  +5.92\\

%ResNet50, SoftNet, ~~$c=0.95$ 
%& 76.62	& 71.96  &  67.82 & 63.94 & 60.48  & 57.57  & 55.39  & 52.94  & 50.67  &  +5.39\\
\bottomrule
\end{tabular}
}
\label{tab:cifar100_5way_5shot_resnet18_20}
\end{center}
% \vspace{-0.1in}
\end{table*}

==> soft-materials/6_exper/5_main_table_ssl.tex <==
\begin{table*}[ht]
\small
\vspace{-0.1in}
\begin{center}
\caption{\small Performance comparison of the proposed method and baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (ACC), average capacity (CAP), and average backward transfer (BWT) across five independent runs. %CF indicates that the method suffers from the catastrophic forgetting. 
The best results are highlighted in bold. Values with $\dagger$ and $\ast$ denote reported performances from \cite{Saha2021} and \cite{Yoon2020}. We consider PackNet~\cite{mallya2018packnet} as the baseline that does not reuse learned weights from past tasks, unlike our WSN.}

\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}}&\multicolumn{3}{c}{\textbf{Permuted MNIST}}&
\multicolumn{3}{c}{\textbf{5 Datasets}}&
\multicolumn{3}{c}{\textbf{Omniglot Rotation}} \\


\midrule
&ACC (\%)&CAP (\%)&BWT&
ACC (\%)&CAP (\%)&BWT&
ACC (\%)&CAP (\%)&BWT \\
\midrule
STL&
%% One significant unita
% {97.2}~\scriptsize($\pm$ 0.1)&{$~$ 1,000.0}&-&
% {93.4}~\scriptsize($\pm$ 0.1)&{$~$ 500.0}&-&
% ~{82.1}~\scriptsize($\pm$ 0.1){\scriptsize*}&{$~$ 10,000.0}& - \\
%% Two significant units
{97.37}~\scriptsize($\pm$ 0.01)&{$~$ 1,000.0}&-&
{93.44}~\scriptsize($\pm$ 0.12)&{$~$ 500.0}&-&
~~{82.13}~\scriptsize($\pm$ 0.08)$^\ast$ &{$~$ 10,000.0}& - \\
 \midrule
FINETUNE&
%% One significant unit 
% {78.2}~\scriptsize($\pm$ 0.8)&{$~$ 100.0}&{-0.21}~\scriptsize($\pm$ 0.01)&
% {80.1}~\scriptsize($\pm$ 0.7)&{$~$ 100.0}&{-0.17}~\scriptsize($\pm$ 0.01)&
% {44.5}~\scriptsize($\pm$ 1.7)&{$~$ 100.0}&{-0.45}~\scriptsize($\pm$ 0.02) \\
%% Two significant units
{78.22}~\scriptsize($\pm$ 0.84)&{$~$ 100.0}&{-0.21}~\scriptsize($\pm$ 0.01)&
{80.06}~\scriptsize($\pm$ 0.74)&{$~$ 100.0}&{-0.17}~\scriptsize($\pm$ 0.01)&
{44.48}~\scriptsize($\pm$ 1.68)&{$~$ 100.0}&{-0.45}~\scriptsize($\pm$ 0.02) \\

EWC~\cite{Kirkpatrick2017}&
%% One significant unit 
% {92.0}~\scriptsize($\pm$ 0.6)&~~{100.0}&{-0.03}~\scriptsize($\pm$ 0.00)&
% ~~{88.6}~\scriptsize($\pm$ 0.3)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.04}~\scriptsize($\pm$ 0.01)$^\dagger$&~{68.7}~\scriptsize($\pm$ 1.9){\scriptsize*}&~~~~{100.0}{\scriptsize*}&{-} \\
{92.01}~\scriptsize($\pm$ 0.56)&~~{100.0}&{-0.03}~\scriptsize($\pm$ 0.00)&
~~{88.64}~\scriptsize($\pm$ 0.26)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.04}~\scriptsize($\pm$ 0.01)$^\dagger$&~~{68.66}~\scriptsize($\pm$ 1.92)$^\ast$&~~~~{100.0}$^\ast$&{-} \\

HAT~\cite{Serra2018}&
%% One significant unit
% {-}&{-}&{-}&
% ~~{91.3}~\scriptsize($\pm$ 0.2)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.03}~\scriptsize($\pm$ 0.00)$^\dagger$&
% {-}&{-}&{-} \\
%% Two significant units
{-}&{-}&{-}&
~~{91.32}~\scriptsize($\pm$ 0.18)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.03}~\scriptsize($\pm$ 0.00)$^\dagger$&
{-}&{-}&{-} \\

GPM~\cite{Saha2021}&
%% One significant unit
% {95.0}~\scriptsize($\pm$ 0.1)&{$~$ 100.0}&{-0.02}~\scriptsize($\pm$ 0.01)&
% ~~{91.2}~\scriptsize($\pm$ 0.2)$^\dagger$&{$~$ 100.0}&~~{-0.01}~\scriptsize($\pm$ 0.00)$^\dagger$&
% {85.2}~\scriptsize($\pm$ 0.4)&{$~$ 100.0}&{-0.01}~\scriptsize($\pm$ 0.00) \\
%% Two significant units
{94.96}~\scriptsize($\pm$ 0.07)&{$~$ 100.0}&{-0.02}~\scriptsize($\pm$ 0.01)&
~~{91.22}~\scriptsize($\pm$ 0.20)$^\dagger$&{$~$ 100.0}&~~{-0.01}~\scriptsize($\pm$ 0.00)$^\dagger$&
{85.24}~\scriptsize($\pm$ 0.37)&{$~$ 100.0}&{-0.01}~\scriptsize($\pm$ 0.00) \\

\midrule
PackNet~\cite{mallya2018packnet}&
%% One significant unit
% {96.4}~\scriptsize($\pm$ 0.0)&{$~$ 96.4}&\textbf{0.0}&
% {92.8}~\scriptsize($\pm$ 0.1)&{$~$ 82.8}&\textbf{0.0}&
% {30.7}~\scriptsize($\pm$ 1.5)&{$~$ 399.2}&\textbf{0.0} \\
%% Two significant units
{96.37}~\scriptsize($\pm$ 0.04)&{$~$ 96.38}&\cellcolor{gg}\textbf{0.0}&
{92.81}~\scriptsize($\pm$ 0.12)&{$~$ 82.86}&\cellcolor{gg}\textbf{0.0}&
{30.70}~\scriptsize($\pm$ 1.50)&{$~$ 399.2}&\cellcolor{gg}\textbf{0.0} \\ 
\midrule
WSN, $c=0.03$&% need to add per-task sparsity
%% One significant unit
% {95.0}~\scriptsize($\pm$ 0.1)&\textbf{{$~$ 20.0}~\scriptsize($\pm$ 0.1)}&\textbf{0.0}&
% {90.6}~\scriptsize($\pm$ 0.7)&\textbf{{$~$ 12.1}~\scriptsize($\pm$ 0.1)}&\textbf{0.0}& % 8.7 + 100*(1-0.78)*5/32 = 12.1 $\pm$ 0.082
% {80.7}~\scriptsize($\pm$ 2.6)&\textbf{{$~~~$ 75.9}~\scriptsize($\pm$ 1.3)}&\textbf{0.0} \\ % 7.1 + 100*(1-0.78)*100/32 = 75.9 $\pm$ 1.24
%% Two significant unit
{94.84}~\scriptsize($\pm$ 0.11)&\textbf{{$~$ 19.87}~\scriptsize($\pm$ 0.16)}&\cellcolor{gg}\textbf{0.0}&
{90.57}~\scriptsize($\pm$ 0.65)&\textbf{{$~$ 12.11}~\scriptsize($\pm$ 0.06)}&\cellcolor{gg}\textbf{0.0}& % 8.7 + 100*(1-0.78)*5/32 = 12.1 $\pm$ 0.082
{80.68}~\scriptsize($\pm$ 2.60)&\textbf{{$~~~$ 75.87}~\scriptsize($\pm$ 1.24)}&\cellcolor{gg}\textbf{0.0} \\ % 7.1 + 100*(1-0.78)*100/32 = 75.9 $\pm$ 1.24

WSN, $c=0.05$&% need to add per-task sparsity
%% One significant unit
% {95.6}~\scriptsize($\pm$ 0.2)&{$~$ 26.3}~\scriptsize($\pm$ 0.3)&\textbf{0.0}&
% {91.6}~\scriptsize($\pm$ 0.2)&{$~$ 17.3}~\scriptsize($\pm$ 0.3)&\textbf{0.0}& % 13.8 + 100*(1-0.78)*5/32 = 17.3
% \textbf{{87.3}~\scriptsize($\pm$ 0.7)}&{$~~~$ 79.8}~\scriptsize($\pm$ 1.2)&\textbf{0.0} \\ % 11.1 + 100*(1-0.78)*100/32 = 79.8
%% Two significant units
{95.65}~\scriptsize($\pm$ 0.03)&{$~$ 26.49}~\scriptsize($\pm$ 0.16)&\cellcolor{gg}\textbf{0.0}&
{91.61}~\scriptsize($\pm$ 0.21)&{$~$ 17.26}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& % 13.8 + 100*(1-0.78)*5/32 = 17.3
\textbf{{87.28}~\scriptsize($\pm$ 0.72)}&{$~~~$ 79.85}~\scriptsize($\pm$ 1.19)&\cellcolor{gg}\textbf{0.0} \\ % 11.1 + 100*(1-0.78)*100/32 = 79.8

WSN, $c=0.1$&% need to add per-task sparsity
%% One significant unit
% {96.2}~\scriptsize($\pm$ 0.1)&{$~$ 40.7}~\scriptsize($\pm$ 0.4)&\textbf{0.0}&
% {92.7}~\scriptsize($\pm$ 0.1)&{$~$ 28.0}~\scriptsize($\pm$ 0.3)&\textbf{0.0}& % 24.6 + 100*(1-0.78)*5/32 = 28.0
% {83.1}~\scriptsize($\pm$ 1.6)&{$~~~$ 83.1}~\scriptsize($\pm$ 1.6)&\textbf{0.0} \\ % 14.3 + 100*(1-0.78)*100/32 = 83.1
%% Two significant units
{96.14}~\scriptsize($\pm$ 0.03)&{$~$ 40.41}~\scriptsize($\pm$ 0.54)&\cellcolor{gg}\textbf{0.0}&
{92.67}~\scriptsize($\pm$ 0.12)&{$~$ 28.01}~\scriptsize($\pm$ 0.28)&\cellcolor{gg}\textbf{0.0}& % 24.6 + 100*(1-0.78)*5/32 = 28.0
{83.10}~\scriptsize($\pm$ 1.56)&{$~~~$ 83.08}~\scriptsize($\pm$ 1.61)&\cellcolor{gg}\textbf{0.0} \\ % 14.3 + 100*(1-0.78)*100/32 = 83.1

WSN, $c=0.3$&% need to add per-task sparsity
%% One significant unit
% \textbf{{96.5}~\scriptsize($\pm$ 0.1)}&{$~$ 77.0}~\scriptsize($\pm$ 0.5)&{\textbf{0.0}}& % 70.2 + 100*(1-0.78)*10/32 = 73.6
% {93.2}~\scriptsize($\pm$ 0.3)&{$~$ 62.3}~\scriptsize($\pm$ 0.7)&\textbf{0.0}& % 58.9 + 100*(1-0.78)*5/32 = 62.3
% {81.9}~\scriptsize($\pm$ 1.1)&{$~$ 102.2}~\scriptsize($\pm$ 0.9)&\textbf{0.0} \\ % 33.4 + 100*(1-0.78)*100/32 = 102.2
%% Two significant units
\textbf{{96.41}~\scriptsize($\pm$ 0.07)}&{$~$ 77.73}~\scriptsize($\pm$ 0.36)&{\cellcolor{gg}\textbf{0.0}}& % 70.2 + 100*(1-0.78)*10/32 = 73.6
{93.22}~\scriptsize($\pm$ 0.32)&{$~$ 62.30}~\scriptsize($\pm$ 0.69)&\cellcolor{gg}\textbf{0.0}& % 58.9 + 100*(1-0.78)*5/32 = 62.3
{81.89}~\scriptsize($\pm$ 1.15)&{$~$ ~~102.2}~\scriptsize($\pm$ 0.89)&\cellcolor{gg}\textbf{0.0} \\ % 33.4 + 100*(1-0.78)*100/32 = 102.2

WSN, $c=0.5$&% need to add per-task sparsity
%% One significant unit
% {96.3}~\scriptsize($\pm$ 0.1)&{$~$ 97.8}~\scriptsize($\pm$ 0.3)&\textbf{0.0}& 
% \textbf{{93.4}~\scriptsize($\pm$ 0.1)}&{$~$ 86.1}~\scriptsize($\pm$ 0.6)&\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
% {79.8}~\scriptsize($\pm$ 2.2)&{$~$ 121.2}~\scriptsize($\pm$ 0.5)&\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2
%% Two significant units
{96.24}~\scriptsize($\pm$ 0.11)&{$~$ 98.10}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
\textbf{{93.41}~\scriptsize($\pm$ 0.13)}&{$~$ 86.10}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{79.80}~\scriptsize($\pm$ 2.16)&{$~$ ~~121.2}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2


\midrule
MTL&
~~{96.70~\scriptsize($\pm$ 0.02)$^\dagger$}&~~{100.0}&{-}&
~~{91.54~\scriptsize($\pm$ 0.28)$^\dagger$}&~~{100.0}&{-}&
{81.23~\scriptsize($\pm$ 0.52)}&~~{100.0}&{-} \\
\bottomrule
\end{tabular}}
%\end{adjustbox}
\label{tab:main_table_ssl}
\vspace{-0.2in}
\end{center}
\end{table*}

==> soft-materials/6_exper/5_main_table_ssl_pmnist.tex <==
\begin{table*}[ht]
\small
\vspace{-0.1in}
\begin{center}
\caption{\small Performance comparison of the proposed method and baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (ACC), average capacity (CAP), and average backward transfer (BWT) across five independent runs. %CF indicates that the method suffers from the catastrophic forgetting. 
The best results are highlighted in bold. Values with $\dagger$ and $\ast$ denote reported performances from \cite{Saha2021} and \cite{Yoon2020}. We consider PackNet~\cite{mallya2018packnet} as the baseline that does not reuse learned weights from past tasks, unlike our WSN.}

\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}}&\multicolumn{3}{c}{\textbf{Permuted MNIST-Sup}}&
\multicolumn{3}{c}{\textbf{Permuted MNIST-FlexMatch}}&
\multicolumn{3}{c}{\textbf{Permuted MNIST-Novel}} \\


\midrule
&ACC (\%)&CAP (\%)&BWT&
ACC (\%)&CAP (\%)&BWT&
ACC (\%)&CAP (\%)&BWT \\
\midrule
%STL&
%{97.37}~\scriptsize($\pm$ 0.01)&{$~$ 1,000.0}&-&
%{93.44}~\scriptsize($\pm$ 0.12)&{$~$ 500.0}&-&
%~~{82.13}~\scriptsize($\pm$ 0.08)$^\ast$ &{$~$ 10,000.0}& - \\
% \midrule
%FINETUNE&
%{78.22}~\scriptsize($\pm$ 0.84)&{$~$ 100.0}&{-0.21}~\scriptsize($\pm$ 0.01)&
%{80.06}~\scriptsize($\pm$ 0.74)&{$~$ 100.0}&{-0.17}~\scriptsize($\pm$ 0.01)&
%{44.48}~\scriptsize($\pm$ 1.68)&{$~$ 100.0}&{-0.45}~\scriptsize($\pm$ 0.02) \\

%EWC~\cite{Kirkpatrick2017}&
%{92.01}~\scriptsize($\pm$ 0.56)&~~{100.0}&{-0.03}~\scriptsize($\pm$ 0.00)&
%~~{88.64}~\scriptsize($\pm$ 0.26)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.04}~\scriptsize($\pm$ 0.01)$^\dagger$&~~{68.66}~\scriptsize($\pm$ 1.92)$^\ast$&~~~~{100.0}$^\ast$&{-} \\

%HAT~\cite{Serra2018}&
%{-}&{-}&{-}&
%~~{91.32}~\scriptsize($\pm$ 0.18)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.03}~\scriptsize($\pm$ 0.00)$^\dagger$&
%{-}&{-}&{-} \\

%GPM~\cite{Saha2021}&
%{94.96}~\scriptsize($\pm$ 0.07)&{$~$ 100.0}&{-0.02}~\scriptsize($\pm$ 0.01)&
%~~{91.22}~\scriptsize($\pm$ 0.20)$^\dagger$&{$~$ 100.0}&~~{-0.01}~\scriptsize($\pm$ 0.00)$^\dagger$&
%{85.24}~\scriptsize($\pm$ 0.37)&{$~$ 100.0}&{-0.01}~\scriptsize($\pm$ 0.00) \\

%\midrule
%PackNet~\cite{mallya2018packnet}&
%{96.37}~\scriptsize($\pm$ 0.04)&{$~$ 96.38}&\cellcolor{gg}\textbf{0.0}&
%{92.81}~\scriptsize($\pm$ 0.12)&{$~$ 82.86}&\cellcolor{gg}\textbf{0.0}&
%{30.70}~\scriptsize($\pm$ 1.50)&{$~$ 399.2}&\cellcolor{gg}\textbf{0.0} \\ 
%\midrule
%WSN, $c=0.03$&% need to add per-task sparsity
%{94.84}~\scriptsize($\pm$ 0.11)&\textbf{{$~$ 19.87}~\scriptsize($\pm$ 0.16)}&\cellcolor{gg}\textbf{0.0}&
%{90.57}~\scriptsize($\pm$ 0.65)&\textbf{{$~$ 12.11}~\scriptsize($\pm$ 0.06)}&\cellcolor{gg}\textbf{0.0}& % 8.7 + 100*(1-0.78)*5/32 = 12.1 $\pm$ 0.082
%{80.68}~\scriptsize($\pm$ 2.60)&\textbf{{$~~~$ 75.87}~\scriptsize($\pm$ 1.24)}&\cellcolor{gg}\textbf{0.0} \\ % 7.1 + 100*(1-0.78)*100/32 = 75.9 $\pm$ 1.24

%WSN, $c=0.05$&% need to add per-task sparsity
%{95.65}~\scriptsize($\pm$ 0.03)&{$~$ 26.49}~\scriptsize($\pm$ 0.16)&\cellcolor{gg}\textbf{0.0}&
%{91.61}~\scriptsize($\pm$ 0.21)&{$~$ 17.26}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& % 13.8 + 100*(1-0.78)*5/32 = 17.3
%\textbf{{87.28}~\scriptsize($\pm$ 0.72)}&{$~~~$ 79.85}~\scriptsize($\pm$ 1.19)&\cellcolor{gg}\textbf{0.0} \\ % 11.1 + 100*(1-0.78)*100/32 = 79.8

%WSN, $c=0.1$&% need to add per-task sparsity
%{96.14}~\scriptsize($\pm$ 0.03)&{$~$ 40.41}~\scriptsize($\pm$ 0.54)&\cellcolor{gg}\textbf{0.0}&
%{92.67}~\scriptsize($\pm$ 0.12)&{$~$ 28.01}~\scriptsize($\pm$ %0.28)&\cellcolor{gg}\textbf{0.0}& % 24.6 + 100*(1-0.78)*5/32 = 28.0
%{83.10}~\scriptsize($\pm$ 1.56)&{$~~~$ 83.08}~\scriptsize($\pm$ 1.61)&\cellcolor{gg}\textbf{0.0} \\ % 14.3 + 100*(1-0.78)*100/32 = 83.1

%WSN, $c=0.3$&% need to add per-task sparsity
%\textbf{{96.41}~\scriptsize($\pm$ 0.07)}&{$~$ 77.73}~\scriptsize($\pm$ 0.36)&{\cellcolor{gg}\textbf{0.0}}& % 70.2 + 100*(1-0.78)*10/32 = 73.6
%{93.22}~\scriptsize($\pm$ 0.32)&{$~$ 62.30}~\scriptsize($\pm$ 0.69)&\cellcolor{gg}\textbf{0.0}& % 58.9 + 100*(1-0.78)*5/32 = 62.3
%{81.89}~\scriptsize($\pm$ 1.15)&{$~$ ~~102.2}~\scriptsize($\pm$ 0.89)&\cellcolor{gg}\textbf{0.0} \\ % 33.4 + 100*(1-0.78)*100/32 = 102.2

%WSN, $c=0.5$, $l=0.0K$ &% need to add per-task sparsity
%{-.-}~\scriptsize($\pm$ 0.11)&{$~$ -.-}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}&
%\textbf{{-.-}~\scriptsize($\pm$ -.-)}&{$~$ -.-}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
%{-.-}~\scriptsize($\pm$ 2.16)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2
%\midrule
WSN, $c=0.5$, $l=0.010K$ &% need to add per-task sparsity
{27.06}~\scriptsize($\pm$ 0.11)&{$~$ 80.60}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& 
{16.60}~\scriptsize($\pm$ 0.11)&{$~$ 83.67}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{-.-}~\scriptsize($\pm$ 2.16)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

WSN, $c=0.5$, $l=0.020K$ &% need to add per-task sparsity
{41.91}~\scriptsize($\pm$ 0.11)&{$~$ 89.25}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& 
{22.56}~\scriptsize($\pm$ 0.11)&{$~$ 90.04}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{-.-}~\scriptsize($\pm$ 2.16)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2


WSN, $c=0.5$, $l=0.100K$ &% need to add per-task sparsity
{74.02}~\scriptsize($\pm$ 0.11)&{$~$ 89.25}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& 
{73.45}~\scriptsize($\pm$ 0.11)&{$~$ 93.30}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{-.-}~\scriptsize($\pm$ 2.16)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

\midrule

WSN, $c=0.5$, $l=1.000K$ &% need to add per-task sparsity
{87.54}~\scriptsize($\pm$ 0.11)&{$~$ 90.49}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{88.42}~\scriptsize($\pm$ 0.11)&{$~$ 90.75}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

WSN, $c=0.5$, $l=1.500K$ &% need to add per-task sparsity
{89.31}~\scriptsize($\pm$ 0.11)&{$~$ 89.82}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{89.78}~\scriptsize($\pm$ 0.11)&{$~$ 91.29}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

WSN, $c=0.5$, $l=2.000K$ &% need to add per-task sparsity
{90.02}~\scriptsize($\pm$ 0.11)&{$~$ 91.13}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{90.86}~\scriptsize($\pm$ 0.11)&{$~$ 90.49}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

WSN, $c=0.5$, $l=3.000K$ &% need to add per-task sparsity
{91.81}~\scriptsize($\pm$ 0.11)&{$~$ 90.26}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{92.30}~\scriptsize($\pm$ 0.11)&{$~$ 89.66}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

WSN, $c=0.5$, $l=4.000K$ &% need to add per-task sparsity
{91.89}~\scriptsize($\pm$ 0.11)&{$~$ 91.14}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{92.42}~\scriptsize($\pm$ 0.11)&{$~$ 91.39}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

WSN, $c=0.5$, $l=5.000K$ &% need to add per-task sparsity
{92.61}~\scriptsize($\pm$ 0.11)&{$~$ 91.75}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{92.76}~\scriptsize($\pm$ 0.11)&{$~$ 91.20}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

\midrule
WSN, $c=0.5$, $l=5.400K$ &% need to add per-task sparsity
{96.24}~\scriptsize($\pm$ 0.11)&{$~$ 98.10}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{96.24}~\scriptsize($\pm$ 0.11)&{$~$ 98.10}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ -.-)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2


%\midrule
%MTL&
%~~{96.70~\scriptsize($\pm$ 0.02)$^\dagger$}&~~{100.0}&{-}&
%~~{91.54~\scriptsize($\pm$ 0.28)$^\dagger$}&~~{100.0}&{-}&
%{81.23~\scriptsize($\pm$ 0.52)}&~~{100.0}&{-} \\
\bottomrule
\end{tabular}}
%\end{adjustbox}
\label{tab:main_table_ssl_pmnist}
\vspace{-0.2in}
\end{center}
\end{table*}

==> soft-materials/6_exper/7_ImageNet.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy of Subnetwork on ImageNet Dataset.}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
%\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{9}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\textbf{cRT}}} \\ 
%\cline{2-10}
Method & lr & scheduler & epoch & soft epoch & sparsity $c$ & $\gamma$ & accuracy   \\
\midrule
HardNet & 0.1 & [31, 61] & 90 & - & 0.1    & 1.0 & -.-   \\ 
HardNet & 0.1 & [31, 61] & 90 & - & 0.01   & 1.0 & -.-   \\ 
HardNet & 0.1 & [31, 61] & 90 & - & 0.001  & 1.0 & -.-   \\ 
HardNet & 0.1 & [31, 61] & 90 & - & 0.0001 & 1.0 & -.-   \\ \midrule

SoftNet & 0.1 & [31, 61] & 90 & 80 & 0.1 & 0.99 & -.-   \\ 
SoftNet & 0.1 & [31, 61] & 90 & 85 & 0.1 & 0.99 & -.-   \\ 
SoftNet & 0.1 & [31, 61] & 90 & 87 & 0.1 & 0.99 & -.-   \\ 
SoftNet & 0.1 & [31, 61] & 90 & 89 & 0.1 & 0.99 & -.-   \\ 

\bottomrule
\end{tabular}}
\label{tab:cifar100_5way_5shot}
\end{center}
\end{table*}

==> soft-materials/6_exper/7_main_cifar100_topic_aanet.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy of ResNet18 on CIFAR-100 for 5-way 5-shot incremental learning with the same class split as in TOPIC~\cite{cheraghian2021semantic}. $^\ast$ denotes the results reported from \cite{shi2021overcoming}. $^\dagger$ represents our reproduced results.}

\resizebox{0.8\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{9}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\makecell{\textbf{The gap} \\ \textbf{with cRT}}}} \\ 
\cline{2-10}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &  \\
\midrule
cRT \cite{shi2021overcoming}$^\ast$ & 72.28 & 69.58 & 65.16 & 61.41 & 58.83 & 55.87 & 53.28 & 51.38 & 49.51 \\ \midrule

AANet \cite{liu2021adaptive}$^\dagger$    
& 79.05 & 67.52 & 62.33 & 56.10 & 51.92 & 45.92 & 45.92 &48.38  & 47.21 & -2.30 \\ \midrule


HardNet (WSN), $c=50\%$   
& 78.35	& 74.12 & 70.13 & 65.88 & 62.74 & 59.56 & 57.98 & 56.31 & 54.32 & +4.81 \\

HardNet (WSN), $c=80\%$   
& 79.27	& 75.38 & 71.11 & 66.68 & 63.32 & 60.06 & 58.16 & 56.40 & 54.31 & +4.80 \\

HardNet (WSN), $c=90\%$   
& 79.22	& 74.77 & 70.89 & 66.41 & 62.90 & 59.48 & 58.10 & 56.13 & 53.92 & +4.41 \\

\midrule

SoftNet, ~~$c=50\%$   
& 79.88  & 75.54  & 71.64  & 67.47  & 64.45  & 61.09  & 59.07  & 57.29  & \textbf{55.33}  & \textbf{+5.82} \\

SoftNet, ~~$c=80\%$   
& \textbf{80.33} & \textbf{76.23}  & \textbf{72.19}  &  \textbf{67.83}  &  \textbf{64.64}  &  \textbf{61.39} & \textbf{59.32}  & \textbf{57.37} & 54.94  & +5.43 \\

SoftNet, ~~$c=90\%$   
& 79.97 & 75.75  & 71.76  & 67.36  & 64.09  & 60.91 &  59.07 & 56.94  & 54.76  & +5.25 \\

\bottomrule
\end{tabular}
}
\label{tab:main_cifar100_5way_5shot_resnet18_topic_aanet}
\end{center}
\end{table*}
